Multi-Purpose Aerial Drones for Network Coverage and Package Delivery

Unmanned aerial vehicles (UAVs) have become important in many applications including last-mile deliveries, surveillance and monitoring, and wireless networks. This paper aims to design UAV trajectories that simultaneously perform multiple tasks. We aim to design UAV trajectories that minimize package delivery time, and at the same time provide uniform coverage over a neighborhood area which is needed for applications such as network coverage or surveillance. We first consider multi-task UAVs for a simplified scenario where the neighborhood area is a circular region with the post office located at its center and the houses are assumed to be uniformly distributed on the circle boundary. We propose a trajectory process such that if according to which the drones move, a uniform coverage can be achieved while the delivery efficiency is still preserved. We then consider a more practical scenario in which the delivery destinations are arbitrarily distributed in an arbitrarily-shaped region. We also do not assume any restrictions on the package arrivals. We show that simultaneous uniform coverage and efficient package delivery is possible for such realistic scenarios. This is shown using both rigorous analyses as well as simulations.

==> Background.tex <==
\section{Background}
\label{sec:background}
In this section, we review the concept of general BPP and uniform BPP. 
If a fixed number of points are independently and identically distributed (i.i.d) on a compact set $W \in R^d$, we say the points can be modeled as a general BPP. If these points are distributed uniformly within the same compact set, then we say the points are modeled according to a uniform BPP \cite{haenggi2012stochastic}. 
The authors of work \cite{} assumed that $D$ UAVs at height $H$ are distributed according to a BPP and start their flights following an arbitrary trajectory process, at times $T_1, T_2, ..., T_N$, independently chosen randomly from $(0, \tau )$ according to a given PDF (It is assumed that the trajectory curves are chosen independently from a certain probability space, and are independent from the starting times $T_1, T_2, ..., T_N$). It can be easily seen that at any arbitrary observation time of $t \geq \tau$, the UAVs still follow a general BPP. However, if these UAVs are distributed according to uniform BPP and move according to an arbitrary trajectory, at a given time instant, the UAVs do not necessarily follow a uniform BPP model.



==> Practical_case-1.tex <==
\section{Practical (General) case}
\label{sec:Practical_case}

 In the general scenario, we do not want to impose specific assumptions on the density or location of homes or the distribution of arrival packages. Therefore, this setting can be applied to any neighborhood area.

\subsection{System Model and the Scenario}
 \begin{figure}[htbp]%
	\centering 	
	\includegraphics[width=0.6\columnwidth]{figs/neighborhood_area_practical_case.png} 	
	\caption{Neighborhood areas for Practical case}
	\label{fig:Practicalcasesneighborhood_area} 	
\end{figure}
Figure \ref{fig:Practicalcasesneighborhood_area} shows a typical neighborhood area over which we want to provide a uniform coverage. In this case, the geometry of neighborhood area does not need to be circular and is generally represented by a 2D shape. In addition, the houses are arbitrarily distributed in the neighborhood area, so the distances from the post office to the houses can be any arbitrary value. Again, we consider a multipurpose scenario: We assume that $D$ drones deliver the arriving packages from the post office to $N$ destination houses and at the same time we want to use them in a UCA framework. We assume packages are continuously arriving at the post office center. The only assumption we make (about the probability distributions of the destinations) is that over a period of time, each destination has non-zero probability.
%
%The $X_1, X_2, X_3, ...$ is a sequence of random variables that shows the sequence of coming packages. We say that the $i^{th}$ package must be delivered to the $k^{th}$ house by $X_i= k$, where $k \in \{1, 2, ..., N\}$.
The location of $h^{th}$ house is defined in a three-dimensional (3D) Cartesian coordinate system by $(x_h, y_h, 0)$,  where $1 \leq h \leq N$. Drones fly at a constant altitude $H$ above the ground and the location of the $d^{th}$ drone at time $t$ is shown by $(X_{d}(t), Y_{d}(t), H)$, where $1 \leq d \leq D$.



\subsection{The Algorithm}
Here, we provide the detailed steps and components of the algorithm for the practical case.
\textbf{Division of the area to small cells:}
In this algorithm, referred to as Algorithm 2,  first, we divide the neighborhood area into small regions (cells). We use $A_l$ to refer to these regions where $1 \leq l \leq S$ and $S$ is the number of cells. We assume that $A_l$ is small so that at most one drone can fly over the cell at any time. This assumption is compatible with  the safety concern of drones as well.

\begin{algorithm}
	\begin{algorithmic}[1]
		\footnotesize	
		\Function{DeliveryCost}{$A, D, m, X$}		
		\Inputs{
			$A$ the area should be covered\\
			D drones with average speed \textit{V}\\
			$m$ number-of packages to deliver\\
			$X$ arrival packages which are not uniformly distributed over $1, 2, ..., N$}
		\Output{Total time to deliver $m$ packages ($T_m$)}
		\State Define $V_{MAX}$ and $V_{MIN}$
		\State Divide $A$ into small cells; called these cells $A_1, A_2, ..., A_S$
		\State for each small cells consider coverage probability $p_r\,,\, 1\,< r\,<S$ and initialize it with 0
		\For{\textit{h=1; $h<=N$}}
		\State Generate the straight trajectory between the post office and $h^{th}$ house and called it $PT_h$
		\EndFor
		\For{\textit{l=1; $l<=S$}}
		\If{No $PT$ passes through $A_l$}
		\State Select $PT_h$ which is the closest trajectory to $A_l$
		\State Change $PT_h$ in such a way that it passes  through $A_l$
		\EndIf
		\EndFor
		\For{\textit{j=1; $j<=\frac{m}{D}$}}
		\For{\textit{i=1; $i<=D$}}
		%\State Generate random variable $T_i$ uniform over $(0, \tau)$.		
		\State Assign $((j-1)*D+i)^{th}$ package to $i^{th}$ drone
		\State Assume $h$ is the destination of $((j-1)*D+i)^{th}$ package
		\State foreach region $l$ which $PT_h$ passes through		
		\If{$p_l\,<p^*$}
		\State Set velocity of $i^{th}$ drone to $MAX(V_{MIN},\frac{H_1(PT_h,A_l)}{p^*-p_l})$
		\Else
		\State Set velocity of $i^{th}$ drone to $MIN(V_{MAX},\frac{H_1(PT_h,A_l)}{p^*-p_l})$
		\EndIf
		\State Update $p_l$
		\EndFor
		\EndFor	
		\EndFunction
	\end{algorithmic}
	\caption{Algorithm corresponding to the practical case}% Algorithm of \ref{sec:Practical_case}}
	\label{alg:case2}	
\end{algorithm}


\textbf{Defining Trajectories:} Then, we should define the trajectory paths, $PT_h:\,1\leq h\leq N$, between the post office and the houses in order to deliver the packages with high efficiency and simultaneously provide the uniform coverage. If we were not concerned about the UCA requirement, the most efficient trajectories would be straight lines from post office to the destinations. Nevertheless, to achieve the UCA requirement, we might need to change trajectories slightly: If needed, we change the straight lines between the post office and the houses in a way that all defined small regions are crossed by at least one trajectory. It means that we want to make sure $((\cup_{h=1}^N{PT_h})\cap A_l\,\neq \varnothing)$ for any region $l$, $1 \leq l \leq S$.






\textbf{Uniform Coverage:} Here, we specifically state the requirement for uniform coverage. Consider the time interval $[0,t]$ where packages are continuously being delivered to their destinations. For any cell $l$, define $c_l(t)$ as the total time that cell is covered (i.e., a drone is flying over that region). The coverage ratio up to time $t$ is defined as $p_l(t)=\frac{c_l(t)}{t}$.
For uniform coverage, we require that for all cells $l=1,2,\cdots, S$, we must have
\[ \lim_{t \rightarrow \infty} p_l(t)=p^*,\]
where $p^*$ is the desired coverage probability. It is worth noting that although to have a rigourous proof we state the condition for the limit case, in practice the convergence is very fast as observed in our simulations in Section \ref{sec:result}.


\textbf{Varying Drone Speeds:}  Algorithm 2 is an \emph{adaptive} algorithm, that is, we adjust the velocity of drones when they enter the regions in order to preserve the uniformity in all cells. Intuitively, if the current coverage ratio is less than the desired coverage probability $p^*$ (i.e., $p_l(t)<p^*$), we should decrease the velocity of the drone, and if it is more than the expected coverage probability, the drone should pass this region faster. Lines 21 to 25 of Algorithm~\ref{alg:case2} show this adjustment, where $H_1$ is  Hausdorff measure.

\begin{figure}[htbp]%
	\centering 	
	\includegraphics[width=0.7\columnwidth]{figs/time_axis.png} 	
	\caption{Arrival/depature of drones over time within a cell }
	\label{fig:time_axis} 	
\end{figure}

Below we show that we can adjust the velocities in a way to guarantee $ \lim_{t \rightarrow \infty} p_l(t)=p^*$ for all cells, $A_l$, $l=1,2,\cdots, S$. For notational simplicity, we will sometimes drop the subscript $l$ in the rest of the proof. Define $L$ as $H_1((\cup_{h=1}^N{PT_h})\cap A_l)$, i.e., the lengths of the part of trajectories restricted to cell $l$. Fig.~\ref{fig:time_axis} demonstrates arrival/departure of drones over the region during a delivery period for $m$ packages. As you can see, first the drone arrives over the region at time $t_1$ and traverses the cell with speed $V_1$, and leaves the region at time $t_2$. In general, the  $k^{th}$ drone arrives over the cell at time $t_{2k-1}$ and leaves the region at time $t_{2k}$ (traverses the cell with speed $V_k$). The time between the arrival and departure of the $k^{th}$ drone in cell $l$ is denoted by $\Delta_k$ and the time between departure of the $k^{th}$ drone and arrival of the $(k+1)^{th}$ is shown by $\delta_k$. Thus,
\begin{align*}
\Delta_k=t_{2k}-t_{2k-1}.\\\delta_k=t_{2k+1}-t_{2k}.
\end{align*}
Suppose the maximum and minimum possible speeds of drones are given by $V_{MAX}$ and $V_{MIN}$. If we define $\Delta_{MAX}=\frac{L}{V_{MIN}}$ and $\Delta_{MIN}=\frac{L}{V_{MAX}}$, then we have $0<\Delta_{MIN} \leq \Delta_k \leq \Delta_{MAX}$. In any practical scenarios, the $\delta_k$ values can not be unlimited. So here we assume that there exit $\delta_{MIN} \ge 0$ and $\delta_{MAX} \ge 0$ such that for all $k$, $0<\delta_{MIN} \leq \delta_k \leq \delta_{MAX}$. Before stating and proving the main theorem, we need the following definition.

	\begin{define} (Causal Velocity Profiles)
		An algorithm for determining $V_j$ for $j=1, 2, \dots$ is said to be casual, if the value of $V_j$ is determined only by the past data up-to time $t_{2j-1}$.
	\end{define}

\begin{thm}\label{thm:case2}
If $V_{MIN}$ and $V_{MAX}$ can be chosen such that $V_{MAX} \geq \frac{L(1-p^*)}{p^*\delta_{MIN}}$ and $V_{MIN} \leq \frac{L(1-p^*)}{p^*\delta_{MAX}}$, then there exists a causal velocity profile such that $\lim_{t\to\infty}p_l(t)=p^*$.
\end{thm}
\textit{Note:} This theorem is a main result stating that the UCA requirement can be satisfied. The conditions $V_{MIN}$ and $V_{MAX}$ simply state that we should be able to have a large enough range for the velocities to be able to achieve uniform coverage. The proof is given below. The readers less interested in the technical proof, can refer to Section \ref{sec:result} to see the simulation results showing the performance of the proposed algorithms for two real neighborhood areas: University of Massachusetts Amherst and Union Point, which is a smart city near Boston.

\begin{proof}
	For simplicity, assume only one path goes through $A_l$ (The proof can easily be extended to multiple paths). Since at any time, at most one drone flies over each cell, we can say that $c_l(t_{2k})=\Sigma_{i=1}^k\Delta_k$ and also $c_l(t_{2k+1})=\Sigma_{i=1}^k\Delta_i$. From these expressions, the following equations can be concluded:
	\begin{equation}
	p(t_{2k})=\frac{c(t_{2k})}{t_{2k}}=\frac{\Sigma_{i=1}^k\Delta_i}{t_{1}+\Sigma_{i=1}^k\Delta_i+\Sigma_{i=1}^{k-1}\delta_j}.
	\end{equation}
	\begin{equation}
	p(t_{2k+1})=\frac{c(t_{2k+1})}{t_{2k+1}}=\frac{\Sigma_{i=1}^k\Delta_i}{t_{1}+\Sigma_{i=1}^k(\Delta_i+\delta_i)}.
	\end{equation}
	
	\begin{lem} \label{lem:timegoesinfinity}
		If all drones traverse the cell with maximum speed at any time i.e. $V_j=V_{MAX}$ for all $j$, then $\limsup\limits_{k\rightarrow\infty}p(t_{2k})\leq p^*$ and if all drones traverse the cell with minimum speed at any time i.e. $V_j=V_{MIN}$ for all $j$, then $\liminf\limits_{k\rightarrow\infty}p(t_{2k})\geq p^*$.
	\end{lem}
	\begin{proof}[Proof of Lemma \ref{lem:timegoesinfinity}]
		If all drones pass the cell with the maximum velocity  $V_{MAX}$, it takes $\frac{L}{V_{MAX}}$ to leave the cell and we can obtain the probability coverage as follows:
		\begin{align*}
		P(t_{2k})=\frac{\Sigma_{i=1}^k\Delta_i}{t_{1}+\Sigma_{i=1}^k\Delta_i+\Sigma_{i=1}^{k-1}\delta_j}=\frac{\frac{kL}{V_{MAX}}}{t_1+\frac{kL}{V_{MAX}}+\Sigma_{i=1}^{k-1}\delta_j}=\\\frac{1}{1+\frac{t_1V_{MAX}}{kL}+\frac{V_{MAX}}{kL}\Sigma_{i=1}^{k-1}\delta_j}.
		\end{align*}
		By using $V_{MAX} \geq \frac{L(1-p^*)}{p^*\delta_{MIN}}$, we have
		\begin{align*}
	     \frac{1}{1+\frac{t_1V_{MAX}}{kL}+\frac{V_{MAX}}{kL}\Sigma_{i=1}^{k-1}\delta_j} \leq \frac{1}{1+\frac{t_1V_{MAX}}{kL}+\frac{1-p^*}{p^*\delta_{MIN}}(\frac{1}{k}\Sigma_{i=1}^{k-1}\delta_j)}\\=\frac{1}{1+\frac{t_1V_{MAX}}{kL}+\frac{1-p^*}{p^*}\frac{k-1}{k}(\frac{1}{(k-1)\delta_{MIN}}\Sigma_{i=1}^{k-1}\delta_j)},
		\end{align*}
		and since $(\frac{1}{(k-1)}\Sigma_{i=1}^{k-1}\delta_j) \geq \delta_{MIN}$, we have
		\begin{align*}
		\limsup\limits_{k\rightarrow\infty}p(t_{2k}) \leq \frac{1}{1+\frac{1-p^*}{p^*}1},
		\end{align*}
		and as a result,
		\begin{align*}
		\limsup\limits_{k\rightarrow\infty}p(t_{2k}) \leq p^*.
		\end{align*}
		Thus if all drones traverse the cell with maximum speed at any time, i.e., $V_j=V_{MAX}$ for all $j$, $\limsup\limits_{k\rightarrow\infty}p(t_{2k}) \leq p^*$. Next, we show if $V_j=V_{MIN}$, then $\lim_{t\to\infty}p_l(t)=p^*$. Now we write
		\begin{align*}
		P(t_{2k})=\frac{\Sigma_{i=1}^k\Delta_i}{t_{1}+\Sigma_{i=1}^k\Delta_i+\Sigma_{i=1}^{k-1}\delta_j}=\frac{\frac{kL}{V_{MIN}}}{t_1+\frac{kL}{V_{MIN}}+\Sigma_{i=1}^{k-1}\delta_j}=\\\frac{1}{1+\frac{t_1V_{MIN}}{kL}+\frac{V_{MIN}}{kL}\Sigma_{i=1}^{k-1}\delta_j}.
		\end{align*}
		By using $V_{MIN} \leq \frac{L(1-p^*)}{p^*\delta_{MAX}}$, we have
		\begin{align*}
		\frac{1}{1+\frac{t_1V_{MIN}}{kL}+\frac{V_{MIN}}{kL}\Sigma_{i=1}^{k-1}\delta_j} \geq \frac{1}{1+\frac{t_1V_{MIN}}{kL}+\frac{1-p^*}{p^*\delta_{MAX}}(\frac{1}{k}\Sigma_{i=1}^{k-1}\delta_j)}\\=\frac{1}{1+\frac{t_1V_{MIN}}{kL}+\frac{1-p^*}{p^*}\frac{k-1}{k}(\frac{1}{(k-1)\delta_{MAX}}\Sigma_{i=1}^{k-1}\delta_j)}.
		\end{align*}
		and since $(\frac{L}{(k-1)}\Sigma_{i=1}^{k-1}\delta_j) \leq \delta_{MAX}$, we have
		\begin{align*}
		\liminf\limits_{k\rightarrow\infty}p(t_{2k}) \geq \frac{1}{1+\frac{1-p^*}{p^*}1},
		\end{align*}
		and as a result,
		\begin{align*}
		\liminf\limits_{k\rightarrow\infty}p(t_{2k}) \geq p^*.
		\end{align*}
		Thus if all drones traverse the cell with minimum speed at any time, i.e., $V_j=V_{MIN}$ for all $j$, $\liminf\limits_{k\rightarrow\infty}p(t_{2k}) \geq p^*$.
	\end{proof}
    Note that the above argument can be repeated for the cases where the first $k_0$ values of $V_j$'s are arbitrary as they do not impact the limiting behavior. So we can provide the following corollary. 
	\begin{cor}
	Let $k_0$ be a positive integer. If we have a sequence $V_j$ for $j = 1, 2,\dots , \infty$ such that for all $j \ge k_0$, $V_j = V_{MAX}$, then
	\renewcommand{\theequation}{\Alph{equation}}
	\setcounter{equation}{0}
	\begin{equation}\label{eq:A}
	\begin{aligned}
	\limsup\limits_{k\rightarrow\infty}p(t_{2k}) \leq p^*.
	\end{aligned}
	\end{equation}
	Similarly, If we have a sequence $V_j$ for $j = 1, 2,\dots , \infty$ such that for all $j \ge k_0$, $V_j = V_{MIN}$, then
	\begin{equation}\label{eq:B}
	\begin{aligned}
	\liminf\limits_{k\rightarrow\infty}p(t_{2k})\geq p^*.
	\end{aligned}
	\end{equation}
	\end{cor}
    For the brevity of the notation, let's define $p(t_{2k}, V_{MIN})$ as the value of $p(t_{2k})$ when for all $j \ge k_0$, $V_j = V_{MIN}$, and define $p(t_{2k}, V_{MAX})$, similarly. Thus, we have
    \[ \liminf\limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})\geq p^*.\]
    Now consider two cases: If we have 
    \[ \limsup\limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})\leq p^*,\]
    Then, we will have 
    \[ \lim \limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})= p^*.\]
    Otherwise, we must have
    \[ \limsup\limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})> p^*.\]
    So we have the following corollary.
    \begin{cor} \label{cor:V_MIN}
    For any sequence of $p(t_{2k})$, one of the following is true:
    \[ \lim \limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})= p^*,\]
    Or
    \[ \limsup\limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})> p^*.\]
    \end{cor}
    Similarly
     \begin{cor} \label{cor:V_MAX}
    For any sequence of $p(t_{2k})$, one of the following is true:
    \[ \lim \limits_{k\rightarrow\infty}p(t_{2k}, V_{MAX})= p^*,\]
    Or
    \[ \liminf\limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})< p^*.\]
    \end{cor}
    
    
    
    



	Let's state the following definition which will be used later in Lemma \ref{lem:velocityprogfileexits}.


	\begin{define} (Min-Max Algorithm)
		The min-max algorithm for choosing $V_i$'s is defined as follows: We choose $V_1=V_{MIN}$. For $k \ge 1$, if $p(t_{2k-1})\leq p^*$, then $V_{k}=V_{MIN}$, otherwise $V_{k}=V_{MAX}$.
	\end{define}
 
\begin{lem} \label{lem:updown}
For the min-max algorithm, the following statements are true:
\begin{enumerate}
  \item If $p(t_{2k-1})<p^*$, then $p(t_{2k+1}) \geq p^*$.
  \item If $p(t_{2k-1})>p^*$, then $p(t_{2k+1}) \leq p^*$.
\end{enumerate}
\end{lem}

\begin{proof}
If $p(t_{2k-1})<p^*$, then $V_{k}=V_{MIN}$, so $\Delta_k=\Delta_{MAX}=\frac{L}{V_{MIN}}$.
  	\begin{equation}\label{eq:tk+-1}
	p(t_{2k+1})=\frac{c(t_{2k+1})}{t_{2k+1}}=\frac{c(t_{2k-1})+\Delta_{MAX}}{t_{2k-1}+\Delta_{MAX}+\delta_k}
	\end{equation}
     Now note
     	\begin{equation} \label{eq:DMAXdMAX}
	\frac{\Delta_{MAX}}{\Delta_{MAX}+\delta_k} \geq  \frac{\Delta_{MAX}}{\Delta_{MAX}+\delta_{MAX}} \geq p^*.
	\end{equation}
     The last inequality is the direct result of the main assumption $V_{MIN} \leq \frac{L(1-p^*)}{p^*\delta_{MAX}}$.
     Now by combining $p(t_{2k-1})=\frac{c(t_{2k-1})}{t_{2k-1}}<p^*$ and equations \ref{eq:tk+-1} and \ref{eq:DMAXdMAX}, we conclude $p(t_{2k+1}) \geq p^*$. The second statement of the lemma can be proved similarly.
\end{proof}




\begin{lem} \label{lem:tj+1tj}
We have
$\lim\limits_{j\rightarrow\infty}\left| p(t_{j+1}) - p(t_{j}) \right| = 0$
\end{lem}

\begin{proof}
It suffices to show $\lim\limits_{k\rightarrow\infty}\left| p(t_{2(k+1)}) - p(t_{2k}) \right| = 0$ and $\lim\limits_{k\rightarrow\infty}\left| p(t_{2(k-1)}) - p(t_{2k}) \right| = 0$. The proofs are similar, so we just show the first one. Recall that $P(t_{2k})=\frac{\Sigma_{i=1}^k\Delta_i}{t_{1}+\Sigma_{i=1}^k\Delta_i+\Sigma_{j=1}^{k-1}\delta_j}=\frac{U_k}{W_k}$. Thus, we have $P(t_{2(k+1)})=\frac{U_k+\Delta_{k+1}}{W_k+\Delta_{k+1}+\delta_k}$.
         Remember, that for $\delta_{MIN} \ge 0$ and $\delta_{MAX} \ge 0$, we have for all $k$, $0<\delta_{MIN} \leq \delta_k \leq \delta_{MAX}$ and $0<\Delta_{MIN} \leq \delta_k \leq \Delta_{MAX}$. We have
        \begin{align*}
       	\begin{dcases*}
		k\Delta_{MIN} \leq U_k \leq k\Delta_{MAX}\\
		t_1+ k\Delta_{MIN} + (k-1) \delta_{MIN} \leq W_k \leq t_1+ k\Delta_{MAX} + (k-1) \delta_{MAX}.
		\end{dcases*}
		\end{align*}
Thus, $\lim_{k \rightarrow \infty} U_k=\infty$ and $\lim_{k \rightarrow \infty} W_k=\infty$, and their ratio $\frac{W_k}{U_k}$ is bounded. Therefore, we can conclude that
		\begin{align*}
		\left|p(t_{2(k+1)}) - p(t_{2k})\right| = \frac{\Delta_{k+1}W_k-(\Delta_{k+1}+\delta_k)U_k}{(W_k+\Delta_{k+1}+\delta_k)(W_k)} \to 0
		\end{align*}
		as $k$ goes to infinity.
\end{proof}


	\begin{lem} \label{lem:velocityprogfileexits}
		There exists a casual algorithm $V_j$ for $j = 1, 2,\dots , \infty$ such that
		\renewcommand{\theequation}{\arabic{equation}}
		\setcounter{equation}{11}
		\begin{equation}\label{eq:lemma3}
		\begin{aligned}
		\lim\limits_{j\rightarrow\infty}p(t_{j})= p^*.
		\end{aligned}
		\end{equation}		
	\end{lem}
	\begin{proof}
        Based on Lemma \ref{lem:tj+1tj}, it suffices to show $\lim\limits_{k\rightarrow\infty}p(t_{2k+1})= p^*$.
		There are various choices of velocity profiles $V_j,j=1, 2,\dots,\infty$ that satisfy Equation (\ref{eq:lemma3}). Their differences are in their rate of convergence. The one we have chosen in our algorithm provides a very fast convergence (Figure \ref{alg:case2}). However, for the sake proof, it is easier to use the min-max algorithm defined above.
		
		We claim that using the min-max velocity profile, we can achieve $\lim\limits_{k\rightarrow\infty}p(t_{2k+1})= p^*$. Let $p(t_3) \leq p^*$, then the min-max algorithm adjusts $V_2$ to $V_{MIN}$. In fact, $V_{j+1}$ is tuned to $V_{MIN}$ as long as $p(t_{2j+1}) \leq p^*$. Now, if for all $j>1$, $p(t_{2j+1}, V_{MIN}) \leq p^*$ then by Corollary \ref{cor:V_MIN}, we have $\lim \limits_{k\rightarrow\infty}p(t_{2k+1}, V_{MIN})= p^*$, in which case we are done. Otherwise, there exists a $t_{k_1}$ in which $p(t_{2k_1}+1) \geq p^*$ at which point the algorithm switches to $V_{MAX}$. Similarly, by Corollary \ref{cor:V_MAX}, there exists $t_{k_2} \geq t_{k_1}$ such that $p(t_{2k_2}+1) \leq p^*$, and this oscillation repeats indefinitely (or anytime it stops we are already converging to $p^{*}$ and we are done). Thus, we may assume the sequence $p(t_{2j}+1)$, for $j= 1, 2, \dots$ \textbf{crosses} $p^*$ infinitely many times.





		To complete the proof of Lemma \ref{lem:velocityprogfileexits}, we show that for all $\epsilon > 0$, there exists $k_\epsilon$ such that for all $ k > k_\epsilon$, we have $\left| p(t_{2k+1})-p^* \right| < \epsilon$. First, choose $k_1$ such that for all $k \geq k_1$, we have $ \left| p(t_{2k})-p(t_{2(k-1)}) \right| < \frac{\epsilon}{4}$ and $ \left| p(t_{2k+1})-p(t_{2k-1}) \right| < \frac{\epsilon}{4}$ (Lemma \ref{lem:tj+1tj}).


Without loss of generality assume $p(t_{2k-1})<p^*$. Let $k_\epsilon$ be the smallest $k > k_1$ such that $p(t_{2k_\epsilon+1})$ crosses $p^*$, then we know the following
\begin{enumerate}
  \item $p(t_{2k_\epsilon+1})>p^*$ and $p(t_{2k_\epsilon+3})<p(t_{2k_\epsilon+1})$ (Lemma \ref{lem:updown});
  \item $|p(t_{2k_\epsilon+1})-p^*|<\frac{\epsilon}{2}$;
  \item $|p(t_{2k_\epsilon+3})-p(t_{2k_\epsilon+1})|<\frac{\epsilon}{2}$.
\end{enumerate}
Therefore, we conclude $|p(t_{2k_\epsilon+3})-p^{*}|<\epsilon$. Indeed, repeating the same argument from now on, we conclude for all $ k > k_\epsilon$, we have $\left| p(t_{2k+1})-p^* \right| < \epsilon$.

\end{proof}
	Now we can complete the proof of Theorem \ref{thm:case2}. To do so, we show that the min-max sequence $V_j$ satisfies $\lim_{t\to\infty}p_l(t)=p^*$. It should be noted that we assumed that there exists $\delta_{MIN} > 0$ and $\delta_{MAX} > 0$ such that for all $k$, $0 < \delta_{MIN} \leq \delta_k \leq \delta_{MAX} < \infty $, also there are $\Delta_{MIN} > 0$ and $\Delta_{MAX} > 0$ such that for all $k$, $0 < \Delta_{MIN} \leq \delta_k \leq \Delta_{MAX} < \infty$.
	
	Here, we define $k(t) =min \left(k: t_{2k}\geq t \right)  $. Also, for $t_{2(k-1)} \geq t \geq t_{2k}$ we define the following:
	\begin{align*}
	a_k=\frac{c(t_{2k})}{t_{2k}-\delta_{MAX}-\Delta_{MAX}}\\
	b_k=\frac{c(t_{2(k-1)})}{t_{2(k-1)}+\delta_{MAX}+\Delta_{MAX}}
	\end{align*}
	By using (\ref{eq:lemma3}), we have
	\begin{align*}
	\lim\limits_{k\rightarrow\infty}a_k=\lim\limits_{k\rightarrow\infty}\frac{c(t_{2k})}{t_{2k}-\delta_{MAX}-\Delta_{MAX}}=\lim\limits_{k\rightarrow\infty}\frac{c(t_{2k})}{t_{2k}}\frac{t_{2k}}{t_{2k}-\delta_{MAX}-\Delta_{MAX}}=p^*.	
	\end{align*}
	Similarly, we can conclude that
	\begin{align*}
	\lim\limits_{k\rightarrow\infty}b_k=\lim\limits_{k\rightarrow\infty}\frac{c(t_{2(k-1)})}{t_{2(k-1)}+\delta_{MAX}+\Delta_{MAX}}=\lim\limits_{k\rightarrow\infty}\frac{c(t_{2(k-1)})}{t_{2(k-1)}}\frac{t_{2(k-1)}}{t_{2(k-1)}+\delta_{MAX}+\Delta_{MAX}}=p^*
	\end{align*}
	Using definition of $k(t)$, we have
	\begin{align*}
	p(t) = \frac{c(t)}{t} \leq \frac{c(t_{2k})}{t} \leq \frac{c(t_{2k}))}{t-\delta_{MAX}-\Delta_{MAX}} = a_k\\
	p(t) = \frac{c(t)}{t} \geq \frac{c(t_{2(k-1)})}{t} \geq \frac{c(t_{2(k-1)}))}{t+\delta_{MAX}+\Delta_{MAX}} = b_k
	\end{align*}
	So, for all $t$, we have $b_k(t) \leq p(t) \leq a_k(t)$. Based on this  we can conclude that:
	\begin{align*}
	\begin{dcases*}
	p(t) \geq b_k(t)\\
	p(t) \leq a_k(t)
	\end{dcases*}\Rightarrow\begin{dcases*}
	\liminf\limits_{t\rightarrow\infty}p(t) \geq \liminf\limits_{t\rightarrow\infty}b_k(t) = p^*\\
	\limsup\limits_{t\rightarrow\infty}p(t) \leq \limsup\limits_{t\rightarrow\infty}a_k(t) = p^*(t)
	\end{dcases*}\Rightarrow \lim\limits_{t\rightarrow\infty}p(t)= p^*
	\end{align*}
\end{proof}









































==> Practical_case.tex <==
\section{Practical (General) case}
\label{sec:Practical_case}

 In the general scenario, we do not impose any assumptions on the density or location of homes or the distribution of arrival packages. Therefore, this setting can be applied to any neighborhood area.

\subsection{System Model and the Scenario}
 \begin{figure}[htbp]%
	\centering 	
	\includegraphics[width=0.6\columnwidth]{figs/neighborhood_area_practical_case.png} 	
	\caption{Neighborhood areas for Practical case}
	\label{fig:Practicalcasesneighborhood_area} 	
\end{figure}
Figure \ref{fig:Practicalcasesneighborhood_area} shows a typical neighborhood area over which we want to provide a uniform coverage. In this case, the geometry of neighborhood area does not need to be circular and is generally represented by a 2D shape. In addition, the houses are arbitrarily distributed in the neighborhood area, so the distances from the post office to the houses can be any arbitrary value. Again, we consider a multipurpose scenario: We assume that $D$ drones deliver the arriving packages from the post office to $N$ destination houses and at the same time we want to use them in a UCA framework. We assume packages are continuously arriving at the post office center.
%
%The $X_1, X_2, X_3, ...$ is a sequence of random variables that shows the sequence of coming packages. We say that the $i^{th}$ package must be delivered to the $k^{th}$ house by $X_i= k$, where $k \in \{1, 2, ..., N\}$.
The density of the houses in different points of the neighborhood area is in general non-uniform. The location of $h^{th}$ house is defined in a three-dimensional (3D) Cartesian coordinate system by $(x_h, y_h, 0)$,  where $1 \leq h \leq N$. Drones fly at a constant altitude $H$ above the ground and the location of the $d^{th}$ drone at time $t$ is shown by $(X_{d}(t), Y_{d}(t), H)$, where $1 \leq d \leq D$.



\subsection{The Algorithm}
Here, we provide the detailed steps and component of the algorithm for the practical case.
\textbf{Division of the area to small cells:}
In this algorithm, referred to as Algorithm 2,  first, we divide the neighborhood area into small regions. We use $A_l$ to refer to these regions where $1 \leq l \leq S$ and $S$ is the number of cells. We assume that $A_l$ is small so that at most one drone can fly over the cell at any time. This assumption is compatible with  the safety concern of drones as well.

\begin{algorithm}
	\begin{algorithmic}[1]
		\footnotesize	
		\Function{DeliveryCost}{$A, D, m, X$}		
		\Inputs{
			$A$ the area should be covered\\
			D drones with average speed \textit{V}\\
			$m$ number-of packages to deliver\\
			$X$ arrival packages which are not uniformly distributed over $1, 2, ..., N$}
		\Output{Total time to deliver $m$ packages ($T_m$)}
		\State Define $V_{MAX}$ and $V_{MIN}$
		\State Divide $A$ into small cells; called these cells $A_1, A_2, ..., A_S$
		\State for each small cells consider coverage probability $p_r\,,\, 1\,< r\,<S$ and initialize it with 0
		\For{\textit{h=1; $h<=N$}}
		\State Generate the straight trajectory between the post office and $h^{th}$ house and called it $PT_h$
		\EndFor
		\For{\textit{l=1; $l<=S$}}
		\If{No $PT$ passes through $A_l$}
		\State Select $PT_h$ which is the closest trajectory to $A_l$
		\State Change $PT_h$ in such a way that it passes  through $A_l$
		\EndIf
		\EndFor
		\For{\textit{j=1; $j<=\frac{m}{D}$}}
		\For{\textit{i=1; $i<=D$}}
		%\State Generate random variable $T_i$ uniform over $(0, \tau)$.		
		\State Assign $((j-1)*D+i)^{th}$ package to $i^{th}$ drone
		\State Assume $h$ is the destination of $((j-1)*D+i)^{th}$ package
		\State foreach region $l$ which $PT_h$ passes through		
		\If{$p_l\,<p^*$}
		\State Set velocity of $i^{th}$ drone to $MAX(V_{MIN},\frac{H_1(PT_h,A_l)}{p^*-p_l})$
		\Else
		\State Set velocity of $i^{th}$ drone to $MIN(V_{MAX},\frac{H_1(PT_h,A_l)}{p^*-p_l})$
		\EndIf
		\State Update $p_l$
		\EndFor
		\EndFor	
		\EndFunction
	\end{algorithmic}
	\caption{Algorithm corresponding to the practical case}% Algorithm of \ref{sec:Practical_case}}
	\label{alg:case2}	
\end{algorithm}


Then, we should define the trajectory paths, $PT_h:\,1\leq h\leq N$, between the post office and the houses in order to deliver the packages with high efficiency and simultaneously provide the uniform coverage. If we were not concerned about the UCA requirement, the most efficient trajectories would be straight lines from post office to the destinations.  In order to achieve the UCA goals, we change the straight lines between the post office and the houses in a way that all defined small regions are crossed by at least one trajectory. It means that we want to make sure $((\cup_{h=1}^N{PT_h})\cap A_l\,\neq \varnothing)$ for any region $l$, $1 \leq l \leq S$.






\textbf{Uniform Coverage:} Here, we specifically state the requirement for uniform coverage. Consider the time interval $[0,t]$ where packages are continuously being delivered to their destinations. For any cell $i$, define $c(t)$ as the total time that cell is covered (i.e., a drone is flying over that region). The coverage probability is defined as $p_l(t)=\frac{c_l(t)}{t}$.
For uniform coverage, we require that for all cells $l=1,2,\cdots, S$, we must have
\[ \lim_{t \rightarrow \infty} p_l(t)=p^*,\]
where $p^*$ is the desired coverage probability. It is worth noting that although to have a rigourous proof we state the condition for the limit case, in practice the convergence is very fast as observed in our simulations in Section \ref{sec:result}.


\textbf{Varying Drone Speeds:} We do not want to make any specific assumptions about the probability distributions of the destinations of the packages that arrive at the post office. The only assumption we make is that over a period of time, each destination has non-zero probability. Algorithm 2 is an \emph{adaptive} algorithm, that is the velocity of drones are adjusted as the time progresses to ensure uniform coverage.


Specifically, we adjust the velocity of drones when they enter the regions in order to preserve the uniformity in all cells. Intuitively, if the current coverage probability is less than the expected coverage probability $p^*$ (i.e., $p_l(t)<p^*$), we should decrease the velocity of the drone, and if it is more than the expected coverage probability, the drone should pass this region faster. Lines 21 to 25 of Algorithm~\ref{alg:case2} show this adjustment, where $H_1$ is  Hausdorff measure.

\begin{figure}[htbp]%
	\centering 	
	\includegraphics[width=0.7\columnwidth]{figs/time_axis.png} 	
	\caption{Arrival/depature of drones over time within a cell }
	\label{fig:time_axis} 	
\end{figure}

Below we show that we can adjust the velocities in a way to guarantee $ \lim_{t \rightarrow \infty} p(t)=p^*$. Let us consider a specific $l$th cell, $A_l$. For notational simplicity, we will sometimes drop the subscript $l$ in the rest of the proof. Define $L$ as $H_1((\cup_{h=1}^N{PT_h})\cap A_l)$, i.e., the lengths of the part of trajectories restricted to cell $l$. Fig.~\ref{fig:time_axis} demonstrates arrival/departure of drones over the region during a delivery period for $m$ packages. As you can see, first the drone arrives over the region at time $t_1$ and traverses the cell with speed $V_1$, and leaves the region at time $t_2$. Therefore, we can say that the  $k^{th}$ drone arrives over the cell at time $t_{2k-1}$ and leaves the region at time $t_{2k}$ (traverses the cell with speed $V_k$). The interval between arrival and departure of the $k^{th}$ drone is denoted by $\Delta_k$ and time slot $\delta_k$ is the interval between departure of the $k^{th}$ drone and arrival of the $(k+1)^{th}$ drone where $\Delta_k$ and $\delta_k$ are shown as follows:
\begin{align*}
\Delta_k=t_{2k}-t_{2k-1}.\\\delta_k=t_{2k+1}-t_{2k}.
\end{align*}
Suppose the maximum and minimum possible speeds of drones are given by $V_{MAX}$ and $V_{MIN}$. If we define $\Delta_{MAX}=\frac{L}{V_{MIN}}$ and $\Delta_{MIN}=\frac{L}{V_{MAX}}$, then we have $0<\Delta_{MIN} \leq \delta_k \leq \Delta_{MAX}$.

Here, we would like to make the minimum number of assumptions; nevertheless, in any practical scenarios, the $\delta_k$ values can not be unlimited. So here we assume that there exit $\delta_{MIN} \ge 0$ and $\delta_{MAX} \ge 0$ such that for all $k$, $0<\delta_{MIN} \leq \delta_k \leq \delta_{MAX}$.



\begin{thm}\label{thm:case2}
If $V_{MIN}$ and $V_{MAX}$ can be chosen such that $V_{MAX} \geq \frac{L(1-p^*)}{p^*\delta_{MIN}}$ and $V_{MIN} \leq \frac{L(1-p^*)}{p^*\delta_{MAX}}$, then there exists a velocity profile such that $\lim_{t\to\infty}p_l(t)=p^*$.
\end{thm}
\textit{Note:} This theorem is a main result stating that the UCA requirement can be satisfied. The conditions $V_{MIN}$ and $V_{MAX}$ simply state that we should be able to have a large enough range for the velocities to be able to achieve uniform coverage. The proof is given below. The readers less interested in the technical proof, can refer to Section \ref{sec:result} to see the simulation results showing the performance of the proposed algorithms for two real neighborhood areas: University of Massachusetts Amherst and Union Point, which is a smart city near Boston.

\begin{proof}
	For simplicity, assume only one path goes through $A_l$ (This proof can be extended to multiple paths). Since at any time, at most one drone flies over each cell, we can say that $c_l(t_{2k})=\Sigma_{i=1}^k\Delta_k$ and also $c_l(t_{2k+1})=\Sigma_{i=1}^k\Delta_i$. From these expressions, the following equations can be concluded:
	\begin{equation}
	p(t_{2k})=\frac{c(t_{2k})}{t_{2k}}=\frac{\Sigma_{i=1}^k\Delta_i}{t_{1}+\Sigma_{i=1}^k\Delta_i+\Sigma_{i=1}^{k-1}\delta_j}.
	\end{equation}
	\begin{equation}
	p(t_{2k+1})=\frac{c(t_{2k+1})}{t_{2k+1}}=\frac{\Sigma_{i=1}^k\Delta_i}{t_{1}+\Sigma_{i=1}^k(\Delta_i+\delta_i)}.
	\end{equation}
	Before providing the proof, we present the following lemma which will be used later in the proof procedure.
	\begin{lem} \label{lem:timegoesinfinity}
		If all drones traverse the cell with maximum speed at any time i.e. $V_j=V_{MAX}$ for all $j$, then $\limsup\limits_{k\rightarrow\infty}p(t_{2k})\leq p^*$ and if all drones traverse the cell with minimum speed at any time i.e. $V_j=V_{MIN}$ for all $j$, then $\liminf\limits_{k\rightarrow\infty}p(t_{2k})\geq p^*$.
	\end{lem}
	\begin{proof}[Proof of Lemma \ref{lem:timegoesinfinity}]
		If all drones pass the cell with the maximum velocity  $V_{MAX}$, it takes $\frac{L}{V_{MAX}}$ to leave the cell and we can obtain the probability coverage as follows:
		\begin{align*}
		P(t_{2k})=\frac{\Sigma_{i=1}^k\Delta_i}{t_{1}+\Sigma_{i=1}^k\Delta_i+\Sigma_{i=1}^{k-1}\delta_j}=\frac{\frac{kL}{V_{MAX}}}{t_1+\frac{kL}{V_{MAX}}+\Sigma_{i=1}^{k-1}\delta_j}=\\\frac{1}{1+\frac{t_1V_{MAX}}{kL}+\frac{V_{MAX}}{kL}\Sigma_{i=1}^{k-1}\delta_j}.
		\end{align*}
		By using $V_{MAX} \geq \frac{L(1-p^*)}{p^*\delta_{MIN}}$, we have
		\begin{align*}
	     \frac{1}{1+\frac{t_1V_{MAX}}{kL}+\frac{V_{MAX}}{kL}\Sigma_{i=1}^{k-1}\delta_j} \leq \frac{1}{1+\frac{t_1V_{MAX}}{kL}+\frac{1-p^*}{p^*\delta_{MIN}}(\frac{1}{k}\Sigma_{i=1}^{k-1}\delta_j)}\\=\frac{1}{1+\frac{t_1V_{MAX}}{kL}+\frac{1-p^*}{p^*}\frac{k-1}{k}(\frac{1}{(k-1)\delta_{MIN}}\Sigma_{i=1}^{k-1}\delta_j)},
		\end{align*}
		and since $(\frac{1}{(k-1)}\Sigma_{i=1}^{k-1}\delta_j) \geq \delta_{MIN}$, we have
		\begin{align*}
		\limsup\limits_{k\rightarrow\infty}p(t_{2k}) \leq \frac{1}{1+\frac{1-p^*}{p^*}1},
		\end{align*}
		and as a result,
		\begin{align*}
		\limsup\limits_{k\rightarrow\infty}p(t_{2k}) \leq p^*.
		\end{align*}
		Thus if all drones traverse the cell with maximum speed at any time, i.e., $V_j=V_{MAX}$ for all $j$, $\limsup\limits_{k\rightarrow\infty}p(t_{2k}) \leq p^*$. Next, we show if $V_j=V_{MIN}$, then $\lim_{t\to\infty}p_l(t)=p^*$. Now we write
		\begin{align*}
		P(t_{2k})=\frac{\Sigma_{i=1}^k\Delta_i}{t_{1}+\Sigma_{i=1}^k\Delta_i+\Sigma_{i=1}^{k-1}\delta_j}=\frac{\frac{kL}{V_{MIN}}}{t_1+\frac{kL}{V_{MIN}}+\Sigma_{i=1}^{k-1}\delta_j}=\\\frac{1}{1+\frac{t_1V_{MIN}}{kL}+\frac{V_{MIN}}{kL}\Sigma_{i=1}^{k-1}\delta_j}.
		\end{align*}
		By using $V_{MIN} \leq \frac{L(1-p^*)}{p^*\delta_{MAX}}$, we have
		\begin{align*}
		\frac{1}{1+\frac{t_1V_{MIN}}{kL}+\frac{V_{MIN}}{kL}\Sigma_{i=1}^{k-1}\delta_j} \geq \frac{1}{1+\frac{t_1V_{MIN}}{kL}+\frac{1-p^*}{p^*\delta_{MAX}}(\frac{1}{k}\Sigma_{i=1}^{k-1}\delta_j)}\\=\frac{1}{1+\frac{t_1V_{MIN}}{kL}+\frac{1-p^*}{p^*}\frac{k-1}{k}(\frac{1}{(k-1)\delta_{MAX}}\Sigma_{i=1}^{k-1}\delta_j)}.
		\end{align*}
		and since $(\frac{L}{(k-1)}\Sigma_{i=1}^{k-1}\delta_j) \leq \delta_{MAX}$, we have
		\begin{align*}
		\liminf\limits_{k\rightarrow\infty}p(t_{2k}) \geq \frac{1}{1+\frac{1-p^*}{p^*}1},
		\end{align*}
		and as a result,
		\begin{align*}
		\liminf\limits_{k\rightarrow\infty}p(t_{2k}) \geq p^*.
		\end{align*}
		Thus if all drones traverse the cell with minimum speed at any time, i.e., $V_j=V_{MIN}$ for all $j$, $\liminf\limits_{k\rightarrow\infty}p(t_{2k}) \geq p^*$.
	\end{proof}
    Note that the above argument can be repeated for the cases where the first $k_0$ values of $V_j$'s are arbitrary as they do not impact the limiting behavior. So we can provide the following corollary. 
	\begin{cor}
	Let $k_0$ be a positive integer. If we have a sequence $V_j$ for $j = 1, 2,\dots , \infty$ such that for all $j \ge k_0$, $V_j = V_{MAX}$, then
	\renewcommand{\theequation}{\Alph{equation}}
	\setcounter{equation}{0}
	\begin{equation}\label{eq:A}
	\begin{aligned}
	\limsup\limits_{k\rightarrow\infty}p(t_{2k}) \leq p^*.
	\end{aligned}
	\end{equation}
	Similarly, If we have a sequence $V_j$ for $j = 1, 2,\dots , \infty$ such that for all $j \ge k_0$, $V_j = V_{MIN}$, then
	\begin{equation}\label{eq:B}
	\begin{aligned}
	\liminf\limits_{k\rightarrow\infty}p(t_{2k})\geq p^*.
	\end{aligned}
	\end{equation}
	\end{cor}
    For the brevity of the notation, let's define $p(t_{2k}, V_{MIN})$ to mean the value of $p(t_{2k})$ when for all $j \ge k_0$, $V_j = V_{MIN}$, and define $p(t_{2k}, V_{MAX})$, similarly. Thus, we have
    \[ \liminf\limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})\geq p^*.\]
    Now consider two cases: If we have 
    \[ \limsup\limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})\leq p^*,\]
    Then, we will have 
    \[ \lim \limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})= p^*.\]
    Otherwise, we must have
    \[ \limsup\limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})> p^*.\]
    So we have the following corollary.
    \begin{cor} \label{cor:V_MIN}
    For any sequence of $p(t_{2k})$, one of the following is true:
    \[ \lim \limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})= p^*,\]
    Or
    \[ \limsup\limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})> p^*.\]
    \end{cor}
    Similarly
     \begin{cor} \label{cor:V_MAX}
    For any sequence of $p(t_{2k})$, one of the following is true:
    \[ \lim \limits_{k\rightarrow\infty}p(t_{2k}, V_{MAX})= p^*,\]
    Or
    \[ \liminf\limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})< p^*.\]
    \end{cor}
    
    
    
    



	Let's state the following definition which will be used later in Lemma \ref{lem:velocityprogfileexits}.
	\begin{define}
		An algorithm for determining $V_j$ for $j=1, 2, \dots$ is said to be casual, if the value of $V_j$ is determined only by the past data up-to time $t_{2j-1}$.
	\end{define}

	\begin{define} (Min-Max Algorithm)
		The min-max algorithm for choosing $V_i$'s is defined as follows: We choose $V_1=V_{MIN}$, then for $k \ge 1$, if $p(t_{2k-1})\leq p^*$, then $V_{k}=V_{MIN}$, otherwise $V_{k}=V_{MAX}$.
	\end{define}




	\begin{lem} \label{lem:velocityprogfileexits}
		There exists a casual algorithm $V_j$ for $j = 1, 2,\dots , \infty$ such that
		\renewcommand{\theequation}{\arabic{equation}}
		\setcounter{equation}{11}
		\begin{equation}\label{eq:lemma3}
		\begin{aligned}
		\lim\limits_{k\rightarrow\infty}p(t_{2k})= p^*.
		\end{aligned}
		\end{equation}		
	\end{lem}
	\begin{proof}[Proof of lemma \ref{lem:velocityprogfileexits}]
		There are various choices of velocity profiles $V_j,j=1, 2,\dots,\infty$ that satisfy Equation (\ref{eq:lemma3}). Their differences are in their rate of convergence. The one we have chosen in our algorithm provides a very fast convergence (Figure \ref{alg:case2}). However, for the sake proof, it is easier to use the min-max algorithm defined above.
		
		We claim that with this velocity profile, we can achieve $\lim\limits_{k\rightarrow\infty}p(t_{2k})= p^*$. Let $p(t_2) \leq p^*$, then the above algorithm adjusts $V_2$ to $V_{MIN}$. In fact, $V_{j+1}$ is tuned to $V_{MIN}$ as long as $p(t_{2j}) \leq p^*$. Now, if for all $j>1$, $p(t_{2j}, V_{MIN}) \leq p^*$ then by by Corollary \ref{cor:V_MIN}, we have $\lim \limits_{k\rightarrow\infty}p(t_{2k}, V_{MIN})= p^*$, in which case we are done. Otherwise, there exists a $t_{k_1}$ in which $p(t_{2k_1}) \geq p^*$ at which point the algorithm switches to $V_{MAX}$. Similarly, by Corollary \ref{cor:V_MAX}, there exists $t_{k_2} \geq t_{k_1}$ such that $p(T_{2k_2}) \leq p^*$, and this oscillation repeats indefinitely (or anytime it stops we are already converging to $p^{*}$ and we are done). Thus, we may assume the sequence $p(t_{2j})$, for $j= 1, 2, \dots$ \textbf{crosses} $p^*$ infinitely many times. 


Next, we show that $\lim\limits_{k\rightarrow\infty}\left| p(t_{2(k+1)}) - p(t_{2k}) \right| = 0$. Recall that $P(t_{2k})=\frac{\Sigma_{i=1}^k\Delta_i}{t_{1}+\Sigma_{i=1}^k\Delta_i+\Sigma_{j=1}^{k-1}\delta_j}=\frac{U_k}{W_k}$. Thus, we have $P(t_{2(k+1)})=\frac{U_k+\Delta_{k+1}}{W_k+\Delta_{k+1}+\delta_k}$. 
         Remember, that for $\delta_{MIN} \ge 0$ and $\delta_{MAX} \ge 0$, we have for all $k$, $0<\delta_{MIN} \leq \delta_k \leq \delta_{MAX}$ and $0<\Delta_{MIN} \leq \delta_k \leq \Delta_{MAX}$. We have
        \begin{align*}
       	\begin{dcases*}
		k\Delta_{MIN} \leq U_k \leq k\Delta_{MAX}\\
		t_1+ k\Delta_{MIN} + (k-1) \delta_{MIN} \leq W_k \leq t_1+ k\Delta_{MAX} + (k-1) \delta_{MAX}.
		\end{dcases*}
		\end{align*}
Thus, $\lim_{k \rightarrow \infty} U_k=\infty$ and $\lim_{k \rightarrow \infty} W_k=\infty$, and their ratio $\frac{W_k}{U_k}$ is bounded. Therefore, we can conclude that
		\begin{align*}
		\left|p(t_{2(k+1)}) - p(t_{2k})\right| = \frac{\Delta_{k+1}W_k-(\Delta_{k+1}+\delta_k)U_k}{(W_k+\Delta_{k+1}+\delta_k)(W_k)} \to 0
		\end{align*}
		as $k$ goes to infinity.


		Now, we show that for all $\epsilon > 0$, there exists $k_\epsilon$ such that $ k > k_\epsilon$ satisfies $\left| p(t_{2k})-p^* \right| < \epsilon$. First, choose $k^\prime_{\epsilon}$ such that $ \left| p(t_{2k\prime})-p(t_{2(k\prime-1)}) \right| < \frac{\epsilon}{2}$. Let $k_\epsilon$ be the smallest $k > k^\prime_{\epsilon}$ such that $p(t_{2k_\epsilon})$ crosses $p^*$, then we have  $ \left| p(t_{2(k+1)})-p(t_{2k}) \right| < \epsilon$ for all $k$ greater than $k_\epsilon$.
	\end{proof}
	Now we can complete the proof of Theorem \ref{thm:case2}. To do so we show that there exists a casual sequence $V_j$ for all $j=1, 2, \dots$ such that $\lim_{t\to\infty}p_l(t)=p^*$.
	
	We may choose $V_j$ for $j= 1, 2, \dots$ based on Lemma \ref{lem:velocityprogfileexits}. It should be noted that we assumed that there exists $\delta_{MIN} > 0$ and $\delta_{MAX} > 0$ such that for all $k$, $0 < \delta_{MIN} \leq \delta_k \leq \delta_{MAX} < \infty $, also there are $\Delta_{MIN} > 0$ and $\Delta_{MAX} > 0$ such that for all $k$, $0 < \Delta_{MIN} \leq \delta_k \leq \Delta_{MAX} < \infty$.
	
	Here, we define $k(t) =min \left(k: t_{2k}\geq t \right)  $. Also, for $t_{2(k-1)} \geq t \geq t_{2k}$ we define the following:
	\begin{align*}
	a_k=\frac{f(t_{2k})}{t_{2k}-\delta_{MAX}-\Delta_{MAX}}\\
	b_k=\frac{f(t_{2(k-1)})}{t_{2(k-1)}+\delta_{MAX}+\Delta_{MAX}}
	\end{align*}
	By using (\ref{eq:lemma3}), we have
	\begin{align*}
	\lim\limits_{k\rightarrow\infty}a_k=\lim\limits_{k\rightarrow\infty}\frac{f(t_{2k})}{t_{2k}-\delta_{MAX}-\Delta_{MAX}}=\lim\limits_{k\rightarrow\infty}\frac{f(t_{2k})}{t_{2k}}\frac{t_{2k}}{t_{2k}-\delta_{MAX}-\Delta_{MAX}}=p^*.	
	\end{align*}
	Similarly, we can conclude that
	\begin{align*}
	\lim\limits_{k\rightarrow\infty}b_k=\lim\limits_{k\rightarrow\infty}\frac{f(t_{2(k-1)})}{t_{2(k-1)}+\delta_{MAX}+\Delta_{MAX}}=\lim\limits_{k\rightarrow\infty}\frac{f(t_{2(k-1)})}{t_{2(k-1)}}\frac{t_{2(k-1)}}{t_{2(k-1)}+\delta_{MAX}+\Delta_{MAX}}=p^*
	\end{align*}
	Using definition of $k(t)$, we have
	\begin{align*}
	p(t) = \frac{f(t)}{t} \leq \frac{f(t_{2k})}{t} \leq \frac{f(t_{2k}))}{t-\delta_{MAX}-\Delta_{MAX}} = a_k\\
	p(t) = \frac{f(t)}{t} \geq \frac{f(t_{2(k-1)})}{t} \geq \frac{f(t_{2(k-1)}))}{t+\delta_{MAX}+\Delta_{MAX}} = b_k
	\end{align*}
	So, for all $t$, we have $b_k(t) \leq p(t) \leq a_k(t)$. Based on this  we can conclude that:
	\begin{align*}
	\begin{dcases*}
	p(t) \geq b_k(t)\\
	p(t) \leq a_k(t)
	\end{dcases*}\Rightarrow\begin{dcases*}
	\liminf\limits_{t\rightarrow\infty}p(t) \geq \liminf\limits_{t\rightarrow\infty}b_k(t) = p^*\\
	\limsup\limits_{t\rightarrow\infty}p(t) \leq \limsup\limits_{t\rightarrow\infty}a_k(t) = p^*(t)
	\end{dcases*}\Rightarrow \lim\limits_{t\rightarrow\infty}p(t)= p^*
	\end{align*}
\end{proof}









































==> algorithms.tex <==
\section{ Trajectory Process and Algorithms}
\label{sec:algorithm}
In this section, we define four scenarios and provide scheduling and path planning algorithms for the multi-task drones to provide package delivery and uniform network coverage at the same time. We aim to define algorithms for four different scenarios such that if the drones move, the points remain to follow BPP at any time instant, leading to an almost uniform coverage. We show that for all four proposed scenarios at any snapshot of $t$, once all $D$ drones are on air, they can provide uniform network coverage and at the same time they can provide package delivery with high efficiency.

%%%%%%%%%%%%%%%%%%%%%%
In the rest of this section we explain each scenario and show that at any snapshot of $t$, once all $D$ drones are on air, they are BPP distributed and can provide uniform coverage, also at the same time they provide package delivery with high efficiency. In the explanation of trajectory processes, the location of $h^{th}$ house for the first three cases is shown in Polar coordinate system by $(\rho, \theta_h)$  and for the last case it is defined in Cartesian coordinate system by $(x_h, y_h)$,  where $1 \leq h \leq N$. The location of $d^{th}$ drone at time $t$ for the first three cases is defined by $(R_{d}(t), \theta_{d}(t))$  and for the last case by $(X_{d}(t), Y_{d}(t))$, where $1 \leq d \leq D$ and $\gamma \leq R \leq \rho$. 

%We want to provide an algorithm to deliver the $i^{th}$ package to the destination house $X_i$, where $1 \leq i \leq m$ and $m$ is the number of packages.    

%Assume that $D$ drones start their flights to the random delivery destination ${X_1, X_2, X_3, ..., X_D}$ at times $T_1, T_2, ..., T_D$, independently chosen randomly from $(0, \tau )$ according to a given PDF (Note that it is assumed that the location of drones along the delivery path are independent from the starting times $T_1, T_2, ..., T_N$ ). It can be easily seen that at any arbitrary observation time of $t'\geq \rho$ , the drones follow a general BPP. 

\subsection{Case 1 (Ideal case)}\label{sec:case1}
\textbf{Scenario}: We assume that $D$ drones deliver the arriving packages from the post office in a circular neighborhood area. Figure \ref{fig:modelparam} shows the parameters of this scenario, where $\gamma$ is the radius of post office center, and $\rho$ is the radius of entire neighborhood area.  $\theta_i$ ($0 \leq \theta_i \leq \theta_{max}$) is the angle of $i^{th}$ house on the perimeter of the circle sector. In case of full circle, $\theta_{max}=2\pi$. We show the whole neighborhood area $A$ by equation \ref{eq:targetarea}. We assume houses are distributed uniformly over the neighborhood edge. We also assume package destinations are uniformly distributed over $1, 2, ..., N$. 

\begin{figure}[htbp]%
	\centering
	\includegraphics[width=0.6\columnwidth]{figs/parameters.jpg}%
	\caption{Parameters of our system model}%
	\label{fig:modelparam}%
\end{figure}

\begin{equation} \label{eq:targetarea}
A= \{(r, \theta): \gamma \leq r \leq \rho; 0 \leq \theta \leq \theta_{max} \}
\end{equation}

\begin{algorithm}
	\begin{algorithmic}[1]
		\Function{DeliveryCost}{$D, m, X$}		
		\Inputs{
			D drones with average speed \textit{V}\\
			$m$ number -of package to deliver\\
			$X$ arrival packages which are not uniformly distributed over $1, 2, ..., N$}
		\Output{Total time to deliver $m$ packages($T_m$)}
		\For{\texttt{<i=1; j<=$D$>}}
		\State Generate random variable $T_i$ uniform over $(0, \tau)$.
		\State Assign $i^{th}$ package to $i^{th}$ drone
		\State $i^{th}$ drone flies at $T_i$ and fly in a straight line with $V_d(t)$ at angle $\theta_i$ 
		\EndFor
		\State j=D+1;
		\While{\texttt{j<=m>}}		
		\State Assign $j^{th}$ package to a free drone ( say $i^{th}$ drone)
		\State $i^{th}$ drone flies right away and fly in a straight line with $V_d(t)$ at angle $\theta_j$				
		\EndWhile
		\EndFunction
	\end{algorithmic}
	\caption{ Algorithm of \ref{sec:case1}}
	\label{alg:case1}	
\end{algorithm}

In this algorithm, first , we choose take off time for drones, $T_1, T_2, ..., T_D$, independently and uniformly from $(0, \tau)$, where $\tau$ is the time needed for one drone to reach the neighborhood edge from post office in a straight line by average velocity ($\tau = \frac{\rho-\gamma}{V_{avg}}$). A package $X_i = k (1 \leq k \leq N, i = 1, 2, ...)$ is assigned to a free drone to be delivered. Each drone first flies to a predetermined altitude of $H$, and flies in a straight line with angle $\theta_k$, which is uniform over $(0, \theta_{max})$, towards the neighbourhood edge. Drone distance to the origin at time $t$ is shown by a random variable $R(t)$. When the drone reaches the neighbourhood edge and delivers its assigned package, it returns to the origin on the same angle to complete the first cycle and this action repeats continuously. We list the assumptions of this trajectory process as follows. Figure~\ref{fig:idealcase} shows this trajectory process.

\begin{figure}[htbp]%
	\centering
	\includegraphics[width=0.5\columnwidth]{figs/idealcase.jpg}%
	\caption{First process trajectory}%
	\label{fig:idealcase}%
\end{figure}

We show that if $d_{th}$ drone's distance from the post office at time $t$ ($R_{d}(t)$) follows the equation~\ref{eq:loccase1}, it will provide the uniformly network coverage over the area $A$.

\begin{equation} \label{eq:loccase1}
R_{d}(t)=\begin{cases}
\sqrt{\frac{(\rho^2 -\gamma^2)(t-T_d)}{\tau}+\gamma^2}, & \text{if $T_d \leq t \leq T_d+\tau$}.\\
\sqrt{\frac{(\rho^2 -\gamma^2)(2\tau+T_d-t)}{\tau}+\gamma^2}, & \text{if $T_d+\tau \leq t \leq T_d+2\tau$}.
\end{cases}
\end{equation}

\begin{thm}\label{thm:case1}
	For trajectory process 1: i) For all $t > \tau$ , the instantaneous locations of the drones along the delivery path ($(\theta_{d}(t), R_{d}(t))$), form a uniform BPP, and ii) the time to deliver $m$ packages is equal or less than $\frac{2m\tau}{D}+\tau$, i.e., $\Tau_m \leq \frac{2m\tau}{D}+\tau$.  
\end{thm} 
Before providing the proof, we present the following lemma which will be used later in the proof procedure.
\begin{lem} \label{lem:CDF_uniformity}
	For any arbitrary observation time of $t > \tau$ , the D drones that move according to (\ref{eq:loccase1}) are uniformly distributed.
\end{lem}
\begin{proof}
	For the $d^{th}$ drone, consider the first cycle of going from the post office to the destination house, and then coming back to the post office. For any arbitrary observation time of $t>T_d$, drone $d$ has flown for time $t-T_d$, where $T_d$ is the take off time of the $d^{th}$ drone. By \ref{eq:loccase1}, we obtain $R_{d}(t)=\sqrt{\frac{(\rho^2 -\gamma^2)(t-T_d-k\tau)}{\tau}+\gamma^2}$ for $T_d+k\tau \leq t \leq T_d+(k+1)\tau$ and even $k$, and obtain $R_{d}(t)=\sqrt{\frac{(\rho^2 -\gamma^2)((k+1)\tau+T_d-t)}{\tau}+\gamma^2}$ for $T_d+k\tau \leq t \leq T_d+(k+1)\tau$ and odd $k$.\\
	Now assume that $T_d+k\tau \leq t \leq T_d+(k+1)\tau$ and $k$ is odd, we have the following:
	
	\begin{equation}\label{eq:CDF_Td}
	\begin{aligned}
	F_{R_d}(r_d) = Pr(R_d(t) \leq r_d) = Pr( \sqrt{\frac{(\rho^2 -\gamma^2)((k+1)\tau+T_d-t)}{\tau}+\gamma^2} \leq r_d)\\= Pr(T_d \leq \frac{\tau(r_d^2-\gamma^2)}{\rho^2-\gamma^2}-(k+1)\tau+t)=Pr(T_d \leq \omega_d)= F_{T_d}(\omega_d),
	\end{aligned}
	\end{equation}
	
	where $F_{T_d}$ is the CDF of $T_d$ and $\omega_d=\frac{\tau(r_d^2-\gamma^2)}{\rho^2-\gamma^2}-(k+1)\tau+t$.\\ 
	Now to obtain the PDF of the $R_d$, we take the derivative of $F_{R_d}$:
	
	\begin{equation}\label{eq:PDF_uniformity}
	\begin{aligned}
	f_{R_d}(r_d)=\frac{dF_{R_d}(r_d)}{dr_d}=\frac{dF_{T_d}(\omega_d)}{dr_d}	=\frac{d}{dr_d}\int_{0}^{\omega_d}\frac{1}{\tau}\\=\frac{d}{dr_d}(\frac{r_d^2-\gamma^2}{\rho^2-\gamma^2}-(k+1)+\frac{t}{\tau})=\frac{2r_d}{\rho^2-\gamma^2},
	\end{aligned}
	\end{equation}
	
	where (\ref{eq:PDF_uniformity}) is obtained from the fact that $T_d\sim U(0,\tau)$.
\end{proof}
Furthermore, the velocity of the drone is obtained by taking derivative of (\ref{eq:loccase1}):

\begin{equation} \label{eq:speedcase1}
V_{d}(t)=\begin{cases}
\frac{(\rho^2 -\gamma^2)}{2\sqrt{\tau((\rho^2 -\gamma^2)(t-T_d)+\tau\gamma^2)}}, & \text{if $T_d \leq t \leq T_d+\tau$}.\\
\frac{-(\rho^2 -\gamma^2)}{2\sqrt{\tau((\rho^2 -\gamma^2)(2\tau+T_d-t)+\tau\gamma^2})}, & \text{if $T_d+\tau \leq t \leq T_d+2\tau$}.
\end{cases}
\end{equation}

Equation (\ref{eq:speedcase1}) demonstrates that when drones are at larger distance from the post office and closer to the houses, their velocity decrease which means that they fly fast near the post office and spends longer time flying at the larger distances (i.e., near the houses) to provide a uniform coverage.\\
%\begin{lem} \label{lem:CDF}
%	Consider a periodic function $g: \Re \rightarrow [0, \infty)$, where $g(t+ \tau)= g(t)$, $\forall t \in \Re$. $F_{R(t)}(r)$ the CDF of the randomly shifted process $R(t) \overset{\Delta}{=}\,g(t - T)$, $T \sim U(0,\tau)$ is
%	obtained by
%	\begin{equation} \label{eq:CDF}
%	F_{R(t)}(r)= \frac{|A|}{\tau}
%	\end{equation}
%	where $|.|$ is the Lebesgue measure of $A$ defined as $A=\{\alpha \in [0, \tau]\,|\,g(\alpha) \geq r \}$
%\end{lem}
%\begin{proof}
%	\begin{equation} \label{eq:prof_CDF}
%	F_{R(t)}(r)= \int_{0}^{\tau}\,Pr(g(t - T)\geq r|T=\alpha)\,f_T(\alpha)\,d\alpha=\\
%	\frac{1}{\tau}\int_{0}^{\tau} 1_{\{g(t-\alpha)\geq\,r\}}d\alpha=\frac{|A|}{\tau}
%	\end{equation}
%	where $A$ is defined as the region in which $g(\alpha)\geq r$ during one period, i.e., $A=\{\alpha \in [0, \tau]\,|\,g(\alpha) \geq r \}$.
%\end{proof}
%\begin{cor}
%	If we have $g(2\tau - t)\,=\,g(t)$, $t\in(0, \tau)$, and $R(t) \overset{\Delta}{=}\,g(t - T)$, $T \sim U(0,\tau)$, we get a similar distribution since $g(t)$ is symmetric with respect to $\tau$.
%\end{cor}
%We now provide the proof for Theorem \ref{thm:case1}.
%\begin{proof}
%	For the proof of Theorem \ref{thm:case1}, we first need to show that for $t > \tau$ , the location of vehicles are independent. This is intuitive, since $\theta_d\sim U(0, \theta_{max})$ and $T_d\sim U(0,\tau)$ both have been chosen
%	independently. Second, we have to show that the locations are uniformly distributed over $B$. To do so, we note that since, $\theta_d\sim U(0, \theta_{max})$, the phase of an arbitrary point on the curve is uniformly distributed between $0$ and $theta_{max}$, i.e. $\angle P_{d(t)}\sim U(0, \theta_{max})$. It only remains to show that the CDF of the distance between the post office and an arbitrary point on the delivery path. i.e. $\|P_{d(t)}\|= r_{d(t)}$, is equal to the distribution corresponding to uniform BPP over $B$. For notational simplicity, we drop index $d$ in the rest of the proof. Let
%	\begin{equation}
%	u(t)\overset{\Delta}{=}\begin{cases}
%	\|P(h^{-1}(t))\|, & \text{$0 \leq t \leq \tau$}.\\
%	\|P(h^{-1}(2\tau-\,t))\|, & \text{$\tau \leq t \leq 2\tau$}.
%	\end{cases}
%	\end{equation}
%\end{proof}
We now provide the proof for Theorem (\ref{thm:case1}).
\begin{proof}
	To prove the first part of Theorem (\ref{thm:case1}), we first need to show that for $t > \tau$ , the location of vehicles are independent. This is intuitive, since $\theta_d\sim U(0, \theta_{max})$ and $T_d\sim U(0,\tau)$ both have been chosen independently. Second, we have to show that the locations are uniformly distributed over $A$. To do so, we note that since, $\theta_d\sim U(0, \theta_{max})$, the angle of the drone is uniformly distributed between $0$ and $\theta_{max}$, i.e. $\angle P_{d}(t)\sim U(0, \theta_{max})$. In addition, by lemma (\ref{lem:CDF_uniformity}) we proved that the location of drone,i.e. $\|P_{d}(t)\|= R_{d}(t)$, are uniformly distributed over $A$. Therefore, drones are distributed according to uniform BPP over $A$.
	
	The proof of the second part of Theorem (\ref{thm:case1}) is easy; as explained before, departure time of the $D$ drones $T_1, T_2, ..., T_D$ are i.i.d. and uniform over $(0, \tau)$, so by time $\tau$, all $D$ drones have departed and by time $3\tau$, they have delivered at least $D$ packages and come back to the post office center. The delivery time of the rest of packages (i.e., $m-D$ packages) is $\frac{2\tau(m-D)}{D}$, which are  simultaneously delivered by the $D$ drones. Therefore, the time to deliver $m$ packages is equal or less than $\frac{2m\tau}{D}+\tau$.  
\end{proof}

%move to result section
\red{As a result of Theorem\ref{thm:case1}, efficiency is defined by equation \ref{eq:efficiencyth1} which indicates that efficiency becomes close to $1$ as $m$ increases.
\begin{equation}\label{eq:efficiencyth1}
\eta \geq \frac{1}{1+\frac{D}{2m}}
\end{equation}}

%removed for now 
%%if we want to add deterministic version
%\subsection{Scenario 2}\label{sec:case2}
%In this case, we assume a non-probabilistic configuration of the first scenario. We assume $i^{th}$ ($i \in 1, 2, ..., D$) drone starts to take off from the neighborhood area center at time $T_i$ ($T_i \in (0,\tau)$) which is defined by Equation (\ref{eq:Tnonrandom}). It picks up a package $x_i = k$, where $i = 1, 2, ...$ and $k$ is uniformly distributed over $1, 2, ..., N$, and flies to a predetermined altitude of $H$.  Then it flies in a straight line with angle $\theta_k$, which is uniform over $(0, \theta_{max})$, towards the neighborhood edge. When the drone reaches the destination and delivers its package, it returns to the origin on the same angle. It does not change the delivery time and the efficiency, but it might change the uniformity. Due to deterministic nature of this trajectory process, we can not provide a rigorous proof about the convergence probability and we will show empirically in  section~\ref{sec:result} that the uniform coverage is confirmed through simulation.
%
%\begin{figure}[htbp]%
%	\centering
%	\includegraphics[width=0.5\columnwidth]{figs/case2.jpg}%
%	\caption{An illustration of flying drones according to second scenario}%
%	\label{fig:case2}%
%\end{figure}

\subsection{Case 2}\label{sec:case2}
\textbf{Scenario}: We assume that $D$ drones deliver the arriving packages from the post office in a circular neighborhood area. In this scenario, we assume a non-uniform distribution for houses. It means that their angles $\theta_1, \theta_2, ..., \theta_N$ have a non-uniform distribution over $(0, \theta_{max})$. Each drone first picks up a package $X_i = k$, where $i = 1, 2, ...$, and $k$ is uniformly distributed over $1, 2, ..., N$, and flies to a predetermined altitude of $H$.


\begin{algorithm}
	\begin{algorithmic}[1]
		\Function{DeliveryCost}{$D, m, X$}		
		\Inputs{
			D drones with average speed \textit{V}\\
			$m$ number -of package to deliver\\
			$X$ arrival packages which are not uniformly distributed over $1, 2, ..., N$}
		\Output{Total time to deliver $m$ packages($T_m$)}
		\For{\texttt{<i=1; j<=$D$>}}
		\State Generate random variable $T_i$ uniform over $(0, \tau)$.
		\State Assign $i^{th}$ package to $i^{th}$ drone
		\State//First approach; Generate random variable $\phi_{i}|X_{i}=k$ over $[\frac{(k-1)\theta_{max}}{N}, \frac{k\theta_{max}}{N}]$
		\State//Second approach; Generate random variable $\phi_{i}$ in such a way that its distribution ($f_k(\phi)$) makes it closer to the $\theta_i$
		\State $i^{th}$ drone flies at $T_i$ and fly in a straight line with $V_d(t)$ at angle $\phi_{i}$ 
		\EndFor
		\State j=D+1;
		\While{\texttt{j<=m}}		
		\State Assign $j^{th}$ package to a free drone ( say $i^{th}$ drone)
		\State//First approach; State Generate random variable $\phi_{i}|X_{j}=k$ over $[\frac{(k-1)\theta_{max}}{N}, \frac{k\theta_{max}}{N}]$
		\State//Second approach; Generate random variable $\phi_{i}$ in such a way that its distribution ($f_k(\phi)$) makes it closer to the $\theta_j$
		\State $i^{th}$ drone flies at $T_i$ and fly in a straight line with $V_d(t)$ at angle $\phi_{i}$ 
		\State $i^{th}$ drone flies right away and fly in a straight line with $V_d(t)$ at angle $\phi_{i}$				
		\EndWhile
		\EndFunction
	\end{algorithmic}
	\caption{ Algorithm of \ref{sec:case2}}
	\label{alg:case2}	
\end{algorithm}

In algorithm \ref{alg:case2}, to provide a uniform coverage over neighborhood area, we generate a random variable $\phi_{i}$ in such a way that its distribution is almost uniform over interval $(0,\theta_{max})$. Then it flies in a straight line with angle $\phi_{i}$ towards the neighborhood edge. When it reaches to the edge of neighborhood, it flies over the edge toward the destination. After delivering, the drone flies back exactly on the same way. It means it flies on the edge of circular area  until reaching the angle $\phi_{i}$. Then, it returns to the post office on the straight line with angle $\phi_{i}$, and this action repeats continuously.

We use two approaches to define variable $\phi_{i}$:   

\textit{First approach:} We generate a random variable $\phi_{i}$ in such a way that the conditional variable $\phi_{i}|x_{i}=k$ be uniform over interval $[\frac{(k-1)\theta_{max}}{N}, \frac{k\theta_{max}}{N}]$.
\begin{lem} \label{lem:phi_uniformity}
	The unconditional distribution $\phi_{i}$ is uniformly distributed over $[0, \theta_{max}]$.
\end{lem}

\begin{proof}
To proof lemma \ref{lem:phi_uniformity} we simply use the Law of Total Probability as follows:
\begin{equation}\label{eq:P_theta}
\begin{aligned}
f_{\Phi}(\phi_i) = \sum_{1}^{N} f_{\Phi}(\phi_i|x_{i}=k)f_X(x_{i}=k)\\
f_{\Phi}(\phi_i) = \sum_{1}^{N} (\frac{N(u(\phi_i-(k-1)\frac{\theta_{max}}{N})-u(\phi_i-k\frac{\theta_{max}}{N}))}{\theta_{max}})(\frac{1}{N})\\
f_{\Phi}(\phi_i)=(\frac{N(u(\phi_i)-u(\phi_i-N\frac{\theta_{max}}{N}))}{\theta_{max}})(\frac{1}{N})\\
f_{\Phi}(\phi_i)=\frac{u(\phi_i)-u(\phi_i-\theta_{max})}{\theta_{max}}
\end{aligned}
\end{equation}
\end{proof}

\textit{Second approach:} In this case, instead of using an interval around the $\theta_k$ and define a uniform variable over it, we make it more concentrated on the $\theta_k$ neighbourhood and generate random variable $\phi_{i}$ in such a way that its distribution ($f_k(\phi)$) makes it closer to the $\theta_k$. By this approach we make more balance the trade off between the package delivery time and the uniform coverage. Similar to the previous model, we can not provide a rigorous proof about the package delivery time and the convergence probability and instead we will show them empirically in Section~\ref{sec:result} through simulation.

Figure~\ref{fig:case2} shows the relation between $\theta_{k}$ and $\phi_{i}$. After drone $i$ flew on a straight line towards the neighbourhood edge with $V_d(t)$(equation \ref{eq:speedcase1}) at angle $\phi_{i}$, it needs to move with the average velocity $V_{avg}$ on the neighbourhood edge to reach the destination house $k$. Due to deterministic nature of the third scenario, we can not provide a rigorous proof about the package delivery time and the convergence probability and we will show them empirically in  section~\ref{sec:result} through simulation.

\begin{figure}[htbp]%
	\centering
	\includegraphics[width=0.5\columnwidth]{figs/case3.jpg}%
	\caption{Third process trajectory}%
	\label{fig:case2}%
\end{figure}



\subsection{Case 3}\label{sec:case3}
\textbf{Scenario}: We assume that $D$ drones deliver the arriving packages from the post office in a circular neighborhood area. In a more practical scenario, we assume a non-uniform distribution of the package destinations which means $X_1, X_2, X_3, ...$ are not uniformly distributed over $1, 2, ..., N$. In addition, a non-uniform distribution is assumed for houses. It means that their angles $\theta_1, \theta_2, ..., \theta_N$ have a non-uniform distribution over $(0, \theta_{max})$. In this scenario, the houses can be the apartment buildings in which the packages are sent these houses more than other flat houses. 

In Algorithm~\ref{alg:systemmodel4}, the arrival packages are added to a fixed-size ($4D$ elements) waiting queue to be delivered. We generate take off time of drones, $T_1, T_2, ..., T_D$, are independently chosen uniformly from $(0, \tau)$. Then, for each drone $d (1 \leq d \leq D)$ we generate a random variable $\phi_{d}$ which has a uniform distribution over interval $(0,\theta_{max})$. 

In the next step, each drone $d$ picks up a package $X_i = k$ from the waiting queue which is closest to it's angle ($\phi_{d}$), where $k$ is not uniformly distributed over $1, 2, ..., N$, and $i = 1, 2, ...$, $d= 1, 2, ..., D$. Then it flies in a straight line towards the neighborhood edge. When it reaches to the edge of neighborhood, it flies over the edge toward the destination. After delivering, the drone flies back exactly on the same way. It means it flies on the edge of circular area  until reaching the angle $\phi_{d}$. Then, it returns to the post office on the straight line with angle $\phi_{d}$, and this action repeats continuously. 

\begin{algorithm}
	\begin{algorithmic}[1]
		\Function{DeliveryCost}{$D, m, X$}		
		\Inputs{
		D drones with average speed \textit{V}\\
		$m$ number of package to deliver\\
		$X$ arrival packages which are not uniformly distributed over $1, 2, ..., N$}
		\Output{Total time to deliver $m$ packages($T_m$)}
		\For{\texttt{<j=1; j<=m>}}
		\State Generate random variable $\phi$ uniform over $(0, \theta_{max})$.
		\State Select $d^{th}$ drone which is not assigned to packages
		\State Consider the first $l$ destinations in the waiting queue: ${\theta_i}_1, {\theta_i}_2, ..., {\theta_i}_l$.
		\State Select destination $\theta_{i_k}$ ($1 \leq i_k \leq l$) which is closest to $\phi$.
		\State Assign the selected package to $d^{th}$ drone		
		\EndFor
		\EndFunction
	\end{algorithmic}
	\caption{ Algorithm of scenario 4.}
	\label{alg:systemmodel4}	
\end{algorithm} 

In algorithm \ref{alg:systemmodel4}, priority of package selection for delivery is minimum distance to $\phi_d$. However, it may make the waiting time to be delivered of some packages, which have arrived long time ago, too long. To solve this problem, we improve this algorithm and give weight to the packages based on their arrival time so that the package selection is based on both minimum distance to $\phi_d$ and arrival time. Algorithm \ref{alg:modsystemmodelimprv4} shows the modified algorithm. 

\begin{algorithm}
	\begin{algorithmic}[1]
		\Function{DeliveryCost}{$D, m, X$}		
			\Inputs{
			D drones with average speed \textit{V}\\
			$m$ number of package to deliver\\
			$X$ arrival packages which are not uniformly distributed over $1, 2, ..., N$}
		\Output{Total time to deliver $m$ packages($T_m$)}
		\Initialize{Waiting-time= zeros(m)}
		\For{\texttt{<j=1; j<=m>}}
		\State Generate random variable $\phi$ uniform over $(0, \theta_{max})$.
		\State Select $d^{th}$ drone which is not assigned to packages
		\State Consider the first $l$ destinations in the  package queue: $\theta_{i_1}, \theta_{i_2}, ..., \theta_{i_l}$
		\If{there exits Waiting-time(1:$l$) $>$ Threshold-wait-time}
		\State Assign this package to $d^{th}$ drone
		\Else 
		\State Select destination $\theta_i$ ($1 \leq i \leq l$) which is closest to $\phi$.
		\State Assign the package to $d^{th}$ drone
		\EndIf
		\State Increase Waiting-time(1:l) except the assigned package
		\EndFor
		\EndFunction
	\end{algorithmic}
	\caption{Modified algorithm of the scenario 4.}
	\label{alg:modsystemmodelimprv4}	
\end{algorithm} 
 
\subsection{Case 4}\label{sec:case4}
\textbf{Scenario}: We assume that $D$ drones deliver the arriving packages from the post office in a neighborhood area with \textit{any any arbitrary geometrical shape}. In a real scenario, the houses are arbitrary distributed over the neighborhood area. We assume a non-uniform distribution of the package destinations which means $X_1, X_2, X_3, ...$ are not uniformly distributed over $1, 2, ..., N$.
 

==> algorithms_-_Copy.tex <==
\section{ Trajectory Process and Algorithms}
\label{sec:algorithm}
In this section, we define four scenarios and provide scheduling and path planning algorithms for the multi-task drones to provide package delivery and uniform network coverage at the same time. We aim to define algorithms for four different scenarios such that if the drones move, the points remain to follow BPP at any time instant, leading to an almost uniform coverage. We show that for all four proposed scenarios at any snapshot of $t$, once all $D$ drones are on air, they can provide uniform network coverage and at the same time they can provide package delivery with high efficiency.\\
%%%%%%%%%%%%%%%%%%%% bring here from system model
As we mentioned in previous section, to compare different algorithms fairly, we assume that all the drones fly with the average velocity of $v = \frac{\rho-\gamma}{\tau}$, where $\tau$ is the initialization time in which all $D$ drones start to take off. Before explaining each scenario and its algorithm, we obtain a lower bound of the total time to deliver $m$ packages by $D$ drones through lemma~\ref{lem:lem-low-Tau}, which is independent from which algorithm is used.
%We want to compare the scenario in which drones perform only package delivery(single purpose) with the scenario in which drones perform package delivery and network coverage (multi-purpose).
$\Tau_m$ indicates the total time to deliver $m$ packages (note that $m>>D$). For simplicity, we ignore the down times such as night time and we just remove them from our analysis. 
\begin{lem} \label{lem:lem-low-Tau}
	The time to deliver $m$ packages ($\Tau_m$) by $D$ drones must satisfy
	\begin{equation}\label{eq:lower_Tau_m}
	\Tau_m \geq \frac{2m\tau}{D}
	\end{equation}
\end{lem}
where $\tau$ and $D$ are as defined above.
\begin{proof}
	We assume each drone carry only one package at a time. $2\tau$ is the average time that a drone takes to deliver a package and come back, so for simultaneously delivering $m$ packages by $D$ drones, $\frac{2\tau m}{d}$ time is needed.  
\end{proof}
%Equation \ref{eq:lower_Tau_m} shows the lower bound of $\Tau_m$ independent of which algorithm is used.
Using equation~\ref{eq:lower_Tau_m}, efficiency of the used package delivery algorithm is defined as follows.
\begin{equation}\label{eq:efficiency}
\eta = \frac{[\frac{2m\tau}{d}]}{\Tau_m},      0 \leq \eta \leq 1
\end{equation}
If $\eta$ is close to $1$, it means that the algorithm is more efficient.\\
%%%%%%%%%%%%%%%%%%%%%%
In the rest of this section we explain each scenario and show that at any snapshot of $t$, once all $D$ drones are on air, they are BPP distributed and can provide uniform coverage, also at the same time they provide package delivery with high efficiency. In explenation of the trajectory processes, we show the location of $h^{th}$ house in Polar coordinate system by $(\rho, \theta_h)$ and the location of $d^{th}$ drone at time $t$ by $(R_{d}(t), \theta_{d}(t))$, where $1 \leq h \leq N$, $1 \leq d \leq D$, and $\gamma \leq R \leq \rho$. 

%We want to provide an algorithm to deliver the $i^{th}$ package to the destination house $X_i$, where $1 \leq i \leq m$ and $m$ is the number of packages.    

%Assume that $D$ drones start their flights to the random delivery destination ${X_1, X_2, X_3, ..., X_D}$ at times $T_1, T_2, ..., T_D$, independently chosen randomly from $(0, \tau )$ according to a given PDF (Note that it is assumed that the location of drones along the delivery path are independent from the starting times $T_1, T_2, ..., T_N$ ). It can be easily seen that at any arbitrary observation time of $t'\geq \rho$ , the drones follow a general BPP. 

\subsection{Scenario 1}\label{sec:case1}
We assume that $D$ drones start to take off from the post office center at random moments $T_1, T_2, ..., T_D$ $\in(0, \tau)$ where $\tau$ is the initialization time in which all $D$ drones start to take off. $T_1, T_2, ..., T_D$ are independently chosen uniformly from $(0, \tau)$. A package $X_i = k (1 \leq k \leq N, i = 1, 2, ...)$ is assigned to a free drone to be delivered. Each drone first flies to a predetermined altitude of $H$, and flies in a straight line with angle $\theta_k$, which is uniform over $(0, \theta_{max})$, towards the neighbourhood edge. Drone distance to the origin at time $t$ is shown by a random variable $R(t)$. When the drone reaches the neighbourhood edge and delivers its assigned package, it returns to the origin on the same angle to complete the first cycle and this action repeats continuously. We list the assumptions of this trajectory process as follows. Figure~\ref{fig:idealcase} shows this trajectory process.

\begin{itemize}
	\item Location of $N$ houses are independently and identically distributed(i.i.d) random variables $(\theta_1, \theta_2, ..., \theta_N)$ which are uniformly distributed over $(0, \theta_{max})$ on the edge of circular neighborhood area with radius $\rho$.
	\item Destination of arrival packages $X_1, X_2, ...$ are independent and identically distributed (i.i.d.) random variables which are chosen uniformly among $\{1, 2, ..., N\}$, where $N$ is the number of houses.
	\item Departure time of the $D$ drones $(T_1, T_2, ..., T_D)$ are independent and identically distributed (i.i.d.) random variables which are chosen uniformly from $(1, \tau)$. 	
\end{itemize}

\begin{figure}[htbp]%
	\centering
	\includegraphics[width=0.5\columnwidth]{figs/idealcase.jpg}%
	\caption{First process trajectory}%
	\label{fig:idealcase}%
\end{figure}

%To deliver $i^{th}$ package, a free drone $d$ ($1 \leq d \leq D$) with closest departure time to the package arrival time is chosen. $d^{th}$ drone picks up the $i^{th}$ package and start to take off at time $T_d$ from the post office center toward the destination house $X_i = k (1 \leq k \leq N)$ at location $(\theta_k, \rho)$ at a predetermined altitude of $H$. So we can show the location of the $d_{th}$ drone at time $t$ by $(\theta_{d}(t) = \theta_k, R_{d}(t))$. 
We show that if $d_{th}$ drone's distance from the post office at time $t$ ($R_{d}(t)$) follows the equation~\ref{eq:loccase1}, it will provide the uniformly network coverage over the area $B$.

\begin{equation} \label{eq:loccase1}
R_{d}(t)=\begin{cases}
\sqrt{\frac{(\rho^2 -\gamma^2)(t-T_d)}{\tau}+\gamma^2}, & \text{if $T_d \leq t \leq T_d+\tau$}.\\
\sqrt{\frac{(\rho^2 -\gamma^2)(2\tau+T_d-t)}{\tau}+\gamma^2}, & \text{if $T_d+\tau \leq t \leq T_d+2\tau$}.
\end{cases}
\end{equation}

\begin{thm}\label{thm:case1}
	For trajectory process 1: i) For all $t > \tau$ , the instantaneous locations of the drones along the delivery path ($(\theta_{d}(t), R_{d}(t))$), form a uniform BPP, and ii) the time to deliver $m$ packages is equal or less than $\frac{2m\tau}{D}+\tau$, i.e., $\Tau_m \leq \frac{2m\tau}{D}+\tau$.  
\end{thm} 
Before providing the proof, we present the following lemma which will be used later in the proof procedure.
\begin{lem} \label{lem:CDF_uniformity}
	For any arbitrary observation time of $t > \tau$ , the D drones that move according to (\ref{eq:loccase1}) are uniformly distributed.
\end{lem}
\begin{proof}
	For the $d^{th}$ drone, consider the first cycle of going from the post office to the destination house, and then coming back to the post office. For any arbitrary observation time of $t>T_d$, drone $d$ has flown for time $t-T_d$, where $T_d$ is the take off time of the $d^{th}$ drone. By \ref{eq:loccase1}, we obtain $R_{d}(t)=\sqrt{\frac{(\rho^2 -\gamma^2)(t-T_d-k\tau)}{\tau}+\gamma^2}$ for $T_d+k\tau \leq t \leq T_d+(k+1)\tau$ and even $k$, and obtain $R_{d}(t)=\sqrt{\frac{(\rho^2 -\gamma^2)((k+1)\tau+T_d-t)}{\tau}+\gamma^2}$ for $T_d+k\tau \leq t \leq T_d+(k+1)\tau$ and odd $k$.\\
	Now assume that $T_d+k\tau \leq t \leq T_d+(k+1)\tau$ and $k$ is odd, we have the following:
	
	\begin{equation}\label{eq:CDF_Td}
	\begin{aligned}
	F_{R_d}(r_d) = Pr(R_d(t) \leq r_d) = Pr( \sqrt{\frac{(\rho^2 -\gamma^2)((k+1)\tau+T_d-t)}{\tau}+\gamma^2} \leq r_d)\\= Pr(T_d \leq \frac{\tau(r_d^2-\gamma^2)}{\rho^2-\gamma^2}-(k+1)\tau+t)=Pr(T_d \leq \omega_d)= F_{T_d}(\omega_d),
	\end{aligned}
	\end{equation}
	
	where $F_{T_d}$ is the CDF of $T_d$ and $\omega_d=\frac{\tau(r_d^2-\gamma^2)}{\rho^2-\gamma^2}-(k+1)\tau+t$.\\ 
	Now to obtain the PDF of the $R_d$, we take the derivative of $F_{R_d}$:
	
	\begin{equation}\label{eq:PDF_uniformity}
	\begin{aligned}
	f_{R_d}(r_d)=\frac{dF_{R_d}(r_d)}{dr_d}=\frac{dF_{T_d}(\omega_d)}{dr_d}	=\frac{d}{dr_d}\int_{0}^{\omega_d}\frac{1}{\tau}\\=\frac{d}{dr_d}(\frac{r_d^2-\gamma^2}{\rho^2-\gamma^2}-(k+1)+\frac{t}{\tau})=\frac{2r_d}{\rho^2-\gamma^2},
	\end{aligned}
	\end{equation}
	
	where (\ref{eq:PDF_uniformity}) is obtained from the fact that $T_d\sim U(0,\tau)$.
\end{proof}
Furthermore, the velocity of the drone is obtained by taking derivative of (\ref{eq:loccase1}):

\begin{equation} \label{eq:speedcase1}
V_{d}(t)=\begin{cases}
\frac{(\rho^2 -\gamma^2)}{2\sqrt{\tau((\rho^2 -\gamma^2)(t-T_d)+\tau\gamma^2)}}, & \text{if $T_d \leq t \leq T_d+\tau$}.\\
\frac{-(\rho^2 -\gamma^2)}{2\sqrt{\tau((\rho^2 -\gamma^2)(2\tau+T_d-t)+\tau\gamma^2})}, & \text{if $T_d+\tau \leq t \leq T_d+2\tau$}.
\end{cases}
\end{equation}

Equation (\ref{eq:speedcase1}) demonstrates that when drones are at larger distance from the post office and closer to the houses, their velocity decrease which means that they fly fast near the post office and spends longer time flying at the larger distances (i.e., near the houses) to provide a uniform coverage.\\
%\begin{lem} \label{lem:CDF}
%	Consider a periodic function $g: \Re \rightarrow [0, \infty)$, where $g(t+ \tau)= g(t)$, $\forall t \in \Re$. $F_{R(t)}(r)$ the CDF of the randomly shifted process $R(t) \overset{\Delta}{=}\,g(t - T)$, $T \sim U(0,\tau)$ is
%	obtained by
%	\begin{equation} \label{eq:CDF}
%	F_{R(t)}(r)= \frac{|A|}{\tau}
%	\end{equation}
%	where $|.|$ is the Lebesgue measure of $A$ defined as $A=\{\alpha \in [0, \tau]\,|\,g(\alpha) \geq r \}$
%\end{lem}
%\begin{proof}
%	\begin{equation} \label{eq:prof_CDF}
%	F_{R(t)}(r)= \int_{0}^{\tau}\,Pr(g(t - T)\geq r|T=\alpha)\,f_T(\alpha)\,d\alpha=\\
%	\frac{1}{\tau}\int_{0}^{\tau} 1_{\{g(t-\alpha)\geq\,r\}}d\alpha=\frac{|A|}{\tau}
%	\end{equation}
%	where $A$ is defined as the region in which $g(\alpha)\geq r$ during one period, i.e., $A=\{\alpha \in [0, \tau]\,|\,g(\alpha) \geq r \}$.
%\end{proof}
%\begin{cor}
%	If we have $g(2\tau - t)\,=\,g(t)$, $t\in(0, \tau)$, and $R(t) \overset{\Delta}{=}\,g(t - T)$, $T \sim U(0,\tau)$, we get a similar distribution since $g(t)$ is symmetric with respect to $\tau$.
%\end{cor}
%We now provide the proof for Theorem \ref{thm:case1}.
%\begin{proof}
%	For the proof of Theorem \ref{thm:case1}, we first need to show that for $t > \tau$ , the location of vehicles are independent. This is intuitive, since $\theta_d\sim U(0, \theta_{max})$ and $T_d\sim U(0,\tau)$ both have been chosen
%	independently. Second, we have to show that the locations are uniformly distributed over $B$. To do so, we note that since, $\theta_d\sim U(0, \theta_{max})$, the phase of an arbitrary point on the curve is uniformly distributed between $0$ and $theta_{max}$, i.e. $\angle P_{d(t)}\sim U(0, \theta_{max})$. It only remains to show that the CDF of the distance between the post office and an arbitrary point on the delivery path. i.e. $\|P_{d(t)}\|= r_{d(t)}$, is equal to the distribution corresponding to uniform BPP over $B$. For notational simplicity, we drop index $d$ in the rest of the proof. Let
%	\begin{equation}
%	u(t)\overset{\Delta}{=}\begin{cases}
%	\|P(h^{-1}(t))\|, & \text{$0 \leq t \leq \tau$}.\\
%	\|P(h^{-1}(2\tau-\,t))\|, & \text{$\tau \leq t \leq 2\tau$}.
%	\end{cases}
%	\end{equation}
%\end{proof}
We now provide the proof for Theorem (\ref{thm:case1}).
\begin{proof}
	To prove the first part of Theorem (\ref{thm:case1}), we first need to show that for $t > \tau$ , the location of vehicles are independent. This is intuitive, since $\theta_d\sim U(0, \theta_{max})$ and $T_d\sim U(0,\tau)$ both have been chosen independently. Second, we have to show that the locations are uniformly distributed over $B$. To do so, we note that since, $\theta_d\sim U(0, \theta_{max})$, the angle of the drone is uniformly distributed between $0$ and $\theta_{max}$, i.e. $\angle P_{d}(t)\sim U(0, \theta_{max})$. In addition, by lemma (\ref{lem:CDF_uniformity}) we proved that the location of drone,i.e. $\|P_{d}(t)\|= R_{d}(t)$, are uniformly distributed over $B$. Therefore, drones are distributed according to uniform BPP over $B$.
	
	The proof of the second part of Theorem (\ref{thm:case1}) is easy; as explained before, departure time of the $D$ drones $T_1, T_2, ..., T_D$ are i.i.d. and uniform over $(0, \tau)$, so by time $\tau$, all $D$ drones have departed and by time $3\tau$, they have delivered at least $D$ packages and come back to the post office center. The delivery time of the rest of packages (i.e., $m-D$ packages) is $\frac{2\tau(m-D)}{D}$, which are  simultaneously delivered by the $D$ drones. Therefore, the time to deliver $m$ packages is equal or less than $\frac{2m\tau}{D}+\tau$.  
\end{proof}

As a result of Theorem\ref{thm:case1}, efficiency is defined by equation \ref{eq:efficiencyth1} which indicates that efficiency becomes close to $1$ as $m$ increases.
\begin{equation}\label{eq:efficiencyth1}
\eta \geq \frac{1}{1+\frac{D}{2m}}
\end{equation}

\subsection{Scenario 2}\label{sec:case2}
In this case, we assume a non-probabilistic configuration of the first scenario. We assume $i^{th}$ ($i \in 1, 2, ..., D$) drone starts to take off from the neighborhood area center at time $T_i$ ($T_i \in (0,\tau)$) which is defined by Equation (\ref{eq:Tnonrandom}). It picks up a package $x_i = k$, where $i = 1, 2, ...$ and $k$ is uniformly distributed over $1, 2, ..., N$, and flies to a predetermined altitude of $H$.  Then it flies in a straight line with angle $\theta_k$, which is uniform over $(0, \theta_{max})$, towards the neighborhood edge. When the drone reaches the destination and delivers its package, it returns to the origin on the same angle. It does not change the delivery time and the efficiency, but it might change the uniformity. Due to deterministic nature of this trajectory process, we can not provide a rigorous proof about the convergence probability and we will show empirically in  section~\ref{sec:result} that the uniform coverage is confirmed through simulation.

\begin{figure}[htbp]%
	\centering
	\includegraphics[width=0.5\columnwidth]{figs/case2.jpg}%
	\caption{An illustration of flying drones according to second scenario}%
	\label{fig:case2}%
\end{figure}

\subsection{Scenario 3}\label{sec:case3}
We consider $D$ drones with take off times $T_1, T_2, ..., T_D$, which are independently chosen uniformly from $(0, \tau)$. In this scenario, we assume a non-uniform distribution for houses. It means that their angles $\theta_1, \theta_2, ..., \theta_N$ have a non-uniform distribution over $(0, \theta_{max})$. Each drone first picks up a package $x_i = k$, where $i = 1, 2, ...$, and $k$ is uniformly distributed over $1, 2, ..., N$, and flies to a predetermined altitude of $H$. 

To provide a uniform coverage over neighborhood area, we generate a random variable $\phi_{i}$ in such a way that its distribution is almost uniform over interval $(0,\theta_{max})$. Then it flies in a straight line with angle $\phi_{i}$ towards the neighborhood edge. When it reaches to the edge of neighborhood, it flies over the edge toward the destination. After delivering, the drone flies back exactly on the same way. It means it flies on the edge of circular area  until reaching the angle $\phi_{i}$. Then, it returns to the post office on the straight line with angle $\phi_{i}$, and this action repeats continuously.

We use two approaches to define variable $\phi_{i}$:   

\textit{First approach:} We generate a random variable $\phi_{i}$ in such a way that the conditional variable $\phi_{i}|x_{i}=k$ be uniform over interval $[\frac{(k-1)\theta_{max}}{N}, \frac{k\theta_{max}}{N}]$.
\begin{lem} \label{lem:phi_uniformity}
	The unconditional distribution $\phi_{i}$ is uniformly distributed over $[0, \theta_{max}]$.
\end{lem}
%%%%????????? 
\begin{proof}
To proof lemma \ref{lem:phi_uniformity} we simply use the Law of Total Probability as follows:
\begin{equation}\label{eq:P_theta}
\begin{aligned}
f_{\Phi}(\phi_i) = \sum_{1}^{N} f_{\Phi}(\phi_i|x_{i}=k)f_X(x_{i}=k)\\
f_{\Phi}(\phi_i) = \sum_{1}^{N} (\frac{N(u(\phi_i-(k-1)\frac{\theta_{max}}{N})-u(\phi_i-k\frac{\theta_{max}}{N}))}{\theta_{max}})(\frac{1}{N})\\
f_{\Phi}(\phi_i)=(\frac{N(u(\phi_i)-u(\phi_i-N\frac{\theta_{max}}{N}))}{\theta_{max}})(\frac{1}{N})\\
f_{\Phi}(\phi_i)=\frac{u(\phi_i)-u(\phi_i-\theta_{max})}{\theta_{max}}
\end{aligned}
\end{equation}
\end{proof}

Figure~\ref{fig:case3} shows the relation between $\theta_{k}$ and $\phi_{i}$. After drone $i$ flew on a straight line towards the neighbourhood edge with angle $\phi_{i}$, it needs to move with the average velocity $v$ on the neighbourhood edge to reach the destination house $k$. Due to deterministic nature of the third scenario, we can not provide a rigorous proof about the package delivery time and the convergence probability and we will show them empirically in  section~\ref{sec:result} through simulation.

\begin{figure}[htbp]%
	\centering
	\includegraphics[width=0.5\columnwidth]{figs/case3.jpg}%
	\caption{Third process trajectory}%
	\label{fig:case3}%
\end{figure}

\textit{Second approach:} In this case, instead of using an interval around the $\theta_k$ and define a uniform variable over it, we make it more concentrated on the $\theta_k$ neighbourhood and generate random variable $\phi_{i}$ in such a way that its distribution ($f_k(\phi)$) makes it closer to the $\theta_k$. By this approach we make more balance the trade off between the package delivery time and the uniform coverage. Similar to the previous model, we can not provide a rigorous proof about the package delivery time and the convergence probability and instead we will show them empirically in Section~\ref{sec:result} through simulation.

\subsection{Scenario 4}\label{sec:case4}
In a practical scenario, we assume a non-uniform distribution of the package destinations which means $X_1, X_2, X_3, ...$ are not uniformly distributed over $1, 2, ..., N$. In addition, a non-uniform distribution is assumed for houses. It means that their angles $\theta_1, \theta_2, ..., \theta_N$ have a non-uniform distribution over $(0, \theta_{max})$. In this scenario the arrival packages are added to a fixed-size ($4D$ elements) waiting queue to be delivered. We consider take off time of drones, $T_1, T_2, ..., T_D$, are independently chosen uniformly from $(0, \tau)$. Then, for each drone $d (1 \leq d \leq D)$ we generate a random variable $\phi_{d}$ which has a uniform distribution over interval $(0,\theta_{max})$. 

In the next step, each drone $d$ picks up a package $x_i = k$ from the waiting queue which is closest to it's angle ($\phi_{d}$), where $k$ is not uniformly distributed over $1, 2, ..., N$, and $i = 1, 2, ...$, $d= 1, 2, ..., D$. Then it flies in a straight line towards the neighborhood edge. When it reaches to the edge of neighborhood, it flies over the edge toward the destination. After delivering, the drone flies back exactly on the same way. It means it flies on the edge of circular area  until reaching the angle $\phi_{d}$. Then, it returns to the post office on the straight line with angle $\phi_{d}$, and this action repeats continuously. We provide these steps in Algorithm~\ref{alg:systemmodel4}.

%\begin{algorithm}
%	\begin{algorithmic}[1]
%		\State Generate random variable $\phi$ uniform over $(0, \theta_{max})$.
%		\State Select the first $l$ packages $X_1, X_2, ..., X_l$ from the arrival package queue.
%		\State Deliver to destination $\theta_i$ ($1 \leq i \leq l$) which is closest to the current $\phi$.
%		\State Update $\phi$ with $\theta_i$ and replace package $i$ with a new package from the arrival queue.
%		\State Go back to step 3 and repeat the steps.
%	\end{algorithmic}
%	\caption{ Algorithm of the trajectory process 4.}
%	\label{alg:systemmodel4}	
%\end{algorithm}
\setcounter{algorithm}{4}
\begin{algorithm}
	\begin{algorithmic}[1]
		\Function{DeliveryCost}{$D, m, X$}		
		\Inputs{
		D drones with average speed \textit{V}\\
		$m$ number of package to deliver\\
		$X$ arrival packages which are not uniformly distributed over $1, 2, ..., N$}
		\Output{Total time to deliver $m$ packages($T_m$)}
		\For{\texttt{<j=1; j<=n>}}
		\State Generate random variable $\phi$ uniform over $(0, \theta_{max})$.
		\State Select $d^{th}$ drone which is not assigned to packages
		\State Consider the first $l$ destinations in the waiting queue: ${\theta_i}_1, {\theta_i}_2, ..., {\theta_i}_l$.
		\State Select destination $\theta_{i_k}$ ($1 \leq i_k \leq l$) which is closest to $\phi$.
		\State Assign the selected package to $d^{th}$ drone		
		\EndFor
		\EndFunction
	\end{algorithmic}
	\caption{ Algorithm of scenario 4.}
	\label{alg:systemmodel4}	
\end{algorithm} 

In algorithm \ref{alg:systemmodel4}, priority of package selection for delivery is minimum distance to $\phi_d$. However, it may make the waiting time to be delivered of some packages, which have arrived long time ago, too long. To solve this problem, we improve this algorithm and give weight to the packages based on their arrival time so that the package selection is based on both minimum distance to $\phi_d$ and arrival time. Algorithm \ref{alg:modsystemmodelimprv4} shows the modified algorithm. 

\begin{algorithm}
	\begin{algorithmic}[1]
		\Function{DeliveryCost}{$D, m, X$}		
			\Inputs{
			D drones with average speed \textit{V}\\
			$m$ number of package to deliver\\
			$X$ arrival packages which are not uniformly distributed over $1, 2, ..., N$}
		\Output{Total time to deliver $m$ packages($T_m$)}
		\Initialize{Waiting-time= zeros(m)}
		\For{\texttt{<j=1; j<=n>}}
		\State Generate random variable $\phi$ uniform over $(0, \theta_{max})$.
		\State Select $d^{th}$ drone which is not assigned to packages
		\State Consider the first $l$ destinations in the  package queue: $\theta_{i_1}, \theta_{i_2}, ..., \theta_{i_l}$
		\If{there exits Waiting-time(1:$l$) $>$ Threshold-wait-time}
		\State Assign this package to $d^{th}$ drone
		\Else 
		\State Select destination $\theta_i$ ($1 \leq i \leq l$) which is closest to $\phi$.
		\State Assign the package to $d^{th}$ drone
		\EndIf
		\State Increase Waiting-time(1:l) except the assigned package
		\EndFor
		\EndFunction
	\end{algorithmic}
	\caption{Modified algorithm of the scenario 4.}
	\label{alg:modsystemmodelimprv4}	
\end{algorithm} 
 

  

==> model_assumption.tex <==
\section{Model assumptions}
\label{sec:system_model}

In this section, we introduce our four different cases that provide uniform network coverage and package delivery with high efficiency. We start from the \textbf{Ideal case} to the \textbf{Real case}. In first three scenarios, the neighborhood area is circular, but they have a different assumption. In the last scenario, the geometric shape of neighborhood area can be any arbitrary 2D shape.  Figure \ref{fig:threecasesneighborhood_area} shows the neighborhood area is a circle and the post office is located at its center. Houses and offices are located on the perimeter of the circle. This geometric shape is used for first three scenarios. Figure \ref{fig:thelastcaseneighborhood_area} shows the 1550-acre Union Point map which contains multiple apartment and condominium residences to around 2000 residents\cite{unionpoint}.

\begin{figure}[htbp]%
	\centering
	\subfloat[Geometric shape of neighborhood area for first three scenarios]{
	\includegraphics[width=0.6\columnwidth]{figs/neighborhood_area.jpg}\label{fig:threecasesneighborhood_area}}\\
	\subfloat[Geometric shape of neighborhood area for the last scenario]{
		\includegraphics[width=0.6\columnwidth]{figs/neighborhood_area2.png}\label{fig:thelastcaseneighborhood_area}}
	\caption{Neighborhood areas for different scenarios}%
	\label{fig:neighborhood_area}%
\end{figure}

We assume that $D$ drones deliver the arriving packages from the post office to the destination houses and at the same time provide network coverage for the entire neighborhood area. There are $N$ houses which are destinations of the arrival packages. We assume packages are continuously arriving at the post office center. $X_1, X_2, X_3, ...$ is a sequence of random variables that shows the arrival of packages, where $X_i= k$ ($k \in \{1, 2, ..., N\}$) means the $i^{th}$ package must be delivered to the $k^{th}$ house. We assume that all the drones fly with the average velocity of $V_{avg}$. We use this assumption to be able to fairly compare different algorithms and scenarios.

To provide uniformity cooverage we use uniform BPP concept\cite{haenggi2012stochastic}. We say the drones can be modeled as a general BPP, if a fixed they are independently and identically distributed (i.i.d) on a compact set $W \in R^d$. If these drones are distributed uniformly over neighborhood area, then we say the drones are modeled according to a uniform BPP. So as one way to approach the uniform coverage, we formulate the trajectory process problem in terms of preserving uniformity. In other words to satisfy this goal, we want to design a trajectory process involving $D$ drones such that at any time greater than a threshold time, the snapshot locations of the location of drones are distributed according to a uniform BPP process over the neighborhood area.

Here we introduce briefly these four scenarios and in the next section we explain their corresponding algorithms.

\textbf{First scenario (Ideal case):} We assume that $D$ drones deliver the arriving packages from the post office in a circular neighborhood area. We assume houses are distributed uniformly over the neighborhood edge. We also assume package destinations are uniformly distributed over $1, 2, ..., N$. For this case, we prove that drones provide uniform coverage probability and at the same time, the efficiency of package delivery algorithm is almost 1.

\textbf{Second scenario (non-uniform distribution of houses):} In this case, we consider $D$ drones deliver the arriving packages from the post office in a circular neighborhood area. We assume houses are distributed non-uniform over the neighborhood edge. Packages are sent to houses uniformly. We propose two algorithms for this scenario which are explained in detail in Section~\ref{sec:algorithm}.

\textbf{Third scenario (non-uniform distribution of houses and destinations):} In a more practical scenario, we assume $D$ drones deliver packages to houses are distributed non-uniformly over the neighborhood edge, and the packages are sent to them non-uniformly, too. This scenario is more practical because in reality, the packages are sent to some houses more than other houses and there are vary density houses in the different location of neighborhood area. We propose \red{two algorithms} for this scenario which we explain in Section~\ref{sec:algorithm}.

\textbf{Fourth scenario (non-uniform distribution of houses and destinations for any arbitrary geometrical shape):} In a practical scenario, we assume $D$ drones deliver packages to houses are distributed over any arbitrary geometrical shape, and the packages are sent to them non-uniformly, too. We simulated the proposed algorithm in a real community map. \textit{The proposed algorithm for this scenario can be applied to any neighborhood communities}. We prove that the probability coverage of this algorithm converges to a target coverage probability.

In the next section, we explain each scenarios and algorithms in which $D$ drones are on air, they can provide uniform network coverage, and at the same time, they can provide package delivery with high efficiency.















































==> reated_work.tex <==
\section{Related Work}\label{sec:related_work}
%%%% ABS
The most significant features of UAVs are their high mobility and low deployment cost, which motivate service providers to carry out extensive experiments for the implementation of UAV-mounted aerial base stations (ABSs) \cite{Zuckerberg2014ConnectingTW}. ABSs are expected to be promising complements to traditional macrocell base stations (MBSs) in some special scenarios. Take hotspot scenario (e.g., sport event, fiesta) as an example, in which the overwhelming requirement of data transmission demand usually last only for a short period. In this case, a small number of temporal ABSs are sufficient to meet this short-time demand and are more beneficial for service providers than settling additional fixed ground base stations (GBSs) because of the capital expenditure (CAPEX) issue \cite{Sharma2016UAVAssistedHN}. %Typical examples also include emergency scenario, in which malfunction occurs in adjacent MBSs due to natural disaster or regional power failure. To reestablish wireless signal coverage in these areas, deploying ABSs usually works more efficiently than either settling new GBSs or fixing original MBSs \cite{Erdelj2017HelpFT}.

Several research directions on ABSs are in place including performance analysis \cite{ono2016wireless,mozaffari2016unmanned,lyu2016cyclical,chetlur2017downlink,zeng2016throughput,sun2019cooperative}, optimal positioning \cite{mozaffari2015drone,lyu2016placement,kalantari2016number,mozaffari2016efficient}, and path planning \cite{mozaffari2017mobile,wu2017joint,lyu2018uav,wu2018joint}. %As far as performance analysis is concerned, [9] investigated the coverage and rate performance of a network using an ABS serving cellular users affected by underlaid device-to-device (D2D) users. 
A throughput-delay trade-off has been considered in a throughput maximum-minimum problem in \cite{lyu2016cyclical} to optimally allocate time to several ground terminals while the ABS is moving along a certain straight line in a cyclical time division manner. 
%Assuming an ABS that relays data between a transmitter and receiver in a circular path, the authors of [5] considered the variable rate protocol implementation to both the transmitter-relay and relay-receiver links in order to investigate outage probability and achievable rate. 
Furthermore, using the tools from the stochastic geometry, \cite{chetlur2017downlink} and \cite{zhang2019spectrum} provided coverage and throughput analysis in a Binomial point process (BPP) and Poisson point process (PPP) modeled networks of static ABSs, respectively.  The performance of flying ABSs was analyzed in \cite{enayati2019moving} with stochastic UAV flying trajectories. The authors considered a mobile network of drones and examined two trajectory processes for the movement of drones in order to preserve the BPP distribution of drones at any time instance, which leads to an almost uniform coverage.%Also, [26] proposed a stochastic model for ABS networks which considers both the ABS-user link and the ABS-backhaul link simultaneously.

%%% package delivery
Apart from providing ad-hoc communication networks, the use of UAVs for deliveries is presented as a way to increase access to inaccessible locations, e.g. geographically remote locations~\cite{tatham2017flying} or locations that becomes difficult to reach after a disaster due to collapsed roads etc. ~\cite{nedjati2016post}. The work in \cite{Scott2017DroneDM} is concerned with creating drone delivery models for health-care to locate a warehouse with supplies and drone nests to complete final delivery.  A recent survey paper on the drone delivery concept is provided in \cite{otto2018optimization}. Flying sidekick traveling salesman problem to find the optimal delivery path is introduced in \cite{Murray2015TheFS}. To solve the problem, they propose a mixed-integer programming (MIP) formulation and consider two simple heuristics. In Other researchers try to improve solution by providing a novel MIP model and some further heuristics \cite{Agatz2018OptimizationAF,Wang2017TheVR,tatham2017flying}. Challenges include legal restrictions~\cite{nedjati2016post}, potential conflicts between UAVs and commercial flights ~\cite{Networksextended}, and the current state of the technology leading to payload and duration limitations ~\cite{rabta2018drone,chowdhury2017drones}.

Despite these endeavors, there has not been any work on multi-purpose aerial drones. In this work, our aim is to design a  trajectory process with different scenarios in which the ABSs move, provide a fairly uniform user coverage can be maintained while deliver the packages to houses. 



==> system_models.tex <==
\section{Scenarios and Algorithms}
\label{sec:system_model}
%Since UAVs can potentially be used for many different applications, an interesting idea is to design UAVs that simultaneously perform multiple tasks. This could significantly improve the efficiency of such systems. Consider a residential area where drones are used as the last-mile delivery tool within the area. Since these drones are already flying all over the area, it would be great if they can also serve as ABSs for the area. However, this means that we might not be able to choose optimal routing and scheduling algorithms for delivery if we want to provide a relatively uniform coverage.
In this section, we explain our system model and introduce our four different scenarios that provide uniform network coverage and package delivery with high efficiency.

\begin{figure}[htbp]%
	\centering
	\includegraphics[width=0.6\columnwidth]{figs/neighborhood_area.jpg}%
	\caption{Circular neighborhood area where the post office is located at the center and houses are located on the perimeter of circle}%
	\label{fig:neighborhood_area}%
\end{figure} 

\begin{figure}[htbp]%
	\centering
	\includegraphics[width=0.6\columnwidth]{figs/parameters.jpg}%
	\caption{Parameters of our system model}%
	\label{fig:modelparam}%
\end{figure}

Figure \ref{fig:neighborhood_area} shows our system model in which the neighborhood area is a circle and the post office is located at its center. Houses and offices are located 
%somewhat uniformly 
on the perimeter of the circle. Drones deliver the arriving packages from the post office to the destination houses and at the same time provide network coverage for the entire neighborhood area. Figure \ref{fig:modelparam} shows the parameters of our system model, where $\gamma$ is the radius of post office center, and $\rho$ is the radius of entire neighborhood area. Assume there are $N$ houses which are destinations of the arrival packages. $\theta_i$ ($0 \leq \theta_i \leq \theta_{max}$) is the angle of $i^{th}$ house on the perimeter of the circle sector. In case of full circle, $\theta_{max}=2\pi$. We show the whole neighborhood area $B$ by equation \ref{eq:targetarea}.

\begin{equation} \label{eq:targetarea}
B= \{(r, \theta): \gamma \leq r \leq \rho; 0 \leq \theta \leq \theta_{max} \}
\end{equation}

We assume packages are continuously arriving at the post office center. $X_1, X_2, X_3, ...$ is a sequence of random variables that shows the arrival of packages, where $X_i= k$ ($k \in \{1, 2, ..., N\}$) means the $i^{th}$ package must be delivered to the $k^{th}$ house. Suppose that there are $D$ drones at the post office to deliver the arrival packages to the destination houses. We assume that all the drones fly with the average velocity of $v$. We use this assumption to be able to fairly compare different algorithms and scenarios. The average time that a drone takes to deliver a package from the post office to a destination is obtained as $\tau = \frac{\rho-\gamma}{v}$, in which we assumes all $D$ drones start to take off.
%All drones start to take off from the neighborhood area center at random moments $T_1, T_2, ..., T_D$, which are independently chosen uniformly from $(0, \tau)$.   
%%%%%%%%%%%%%%%%%%% move this part to the next section
%To compare different algorithms fairly, we consider a fixed value($\tau$) for the time that a drone spends traveling from the edge of post office center on a straight line to the target house.
%%We want to compare the scenario in which drones perform only package delivery(single purpose) with the scenario in which drones perform package delivery and network coverage (multi-purpose).
%We define $\Tau_m$ as a time to deliver $m$ packages (note that $m>>D$). For simplicity, we ignore the down times such as night time and we just remove them from our analysis. 
%\begin{lem} \label{lem:lem-low-Tau}
%	The lower bound of the time to deliver $m$ packages ($\Tau_m$) is defined as follows:
%	\begin{equation}\label{eq:lower_Tau_m}
%	\Tau_m \geq \frac{2m\tau}{d}
%	\end{equation}
%\end{lem}
%\begin{proof}
%	We assume each drone carry only one package at a time. $2\tau$ is the average time that a drone takes to deliver a package and come back, so for simultaneously delivering $m$ packages by $D$ drones, $\frac{2\tau m}{d}$ time is needed.  
%\end{proof}
%Equation \ref{eq:lower_Tau_m} shows the lower bound of $\Tau_m$ independent of which algorithm is used. Using this equation, efficiency of the used package delivery algorithm is defined as follows.
%\begin{equation}\label{eq:efficiency}
%\eta = \frac{[\frac{2m\tau}{d}]}{\Tau_m}
%\end{equation}
%It is obvious that if $\eta$ is close to $1$, it means that the algorithm is more efficient.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The second goal of our multi-purpose drones is to design trajectory processes involving $D$ UAVs, so that they can provide a relatively uniform and sustainable coverage over a given area ($B$), which is useful for the network coverage application and surveillance application. 
%In order to provide the uniform coverage, we know that if a fixed number of points are independently and identically distributed (i.i.d) on a compact set $W \in R^d$, we say the points can be modeled as a general BPP. If these points are distributed uniformly within the same compact set, then we say the points are modeled according to a uniform BPP \cite{haenggi2012stochastic}.
\subsection{General BPP and uniform BPP}
If a fixed number of points are independently and identically distributed (i.i.d) on a compact set $W \in R^d$, we say the points can be modeled as a general BPP. If these points are distributed uniformly within the same compact set, then we say the points are modeled according to a uniform BPP \cite{haenggi2012stochastic}.

%In \cite{chetlur2017downlink} for a network of static ABSs, which are modeled according to uniform BPP, closed-form formulations for coverage are obtained. Such distribution provides fairly uniform coverage across the neighborhood area but as long as the ABSs are static, and if the ABSs start moving, such a uniformity in coverage is not necessarily preserved. Now suppose that $D$ UAVs at height $H$ are distributed according to a BPP and start their flights following an arbitrary trajectory process, at times $T_1, T_2, ..., T_N$, independently chosen randomly from $(0, \tau )$ according to a given PDF. It can be easily seen that at any arbitrary observation time of $t \geq \tau$, the UAVs still follow a general BPP. However, if these ABSs are distributed according to uniform BPP and move according to an arbitrary trajectory, at a given time instant, then ABSs do not necessarily follow a uniform BPP model. \cite{enayati2019moving}.

Based on this concept, if the UAVs are static, a uniform binomial point process (BPP), where drones are uniformly and independently distributed over the area $B$, would seem to be a reasonable choice to provide a relatively uniform coverage as it is considered in most of the available literature. So as one way to approach the uniform coverage, we formulate the trajectory process problem in terms of preserving uniformity. In other words to satisfy this goal, we want to design a trajectory process involving $D$ drones such that at any time $t>\tau$, the snapshot locations of the location of drones are distributed according to a uniform BPP process over the area $B$.

\subsection{Scenario Assumptions}
We propose four scenarios and for all of them we consider a circular neighborhood area with radius $\rho$ as shown in Figure~\ref{fig:neighborhood_area}. Here we introduce these four scenarios and in the next section we explain their corresponding algorithms.

\textbf{First scenario:} We assume that $D$ drones start to take off from the neighborhood area center at random moments $T_1, T_2, ..., T_D$, which are independently chosen uniformly from $(0, \tau)$ where $\tau$ is the initialization time in which all $D$ drones start to take off. We assume houses are distributed uniformly over the neighborhood edge,i.e., $\theta_i$ ($i \in 1, 2, ..., N$),  where $N$ is number of houses, is uniformly distributed over $(0, \theta_{max})$. We also assume package destinations are uniformly distributed over $1, 2, ..., N$.  %$T_1, T_2, ..., T_D$ are independently chosen uniformly from $(0, \tau)$. Each drone first picks up a package $x_i = k$, where $i = 1, 2, ...$, and $k$ is uniformly distributed over $1, 2, ..., N$, and flies to a predetermined altitude of $H$. Then it flies in a straight line with angle $\theta_k$, which is uniform over $(0, \theta_{max})$, towards the neighborhood edge where its distance to the origin at time $t$ is shown by the random variable $R(t)$. When a drone reaches the neighborhood edge and delivers its assigned package, it returns to the origin on the same angle to complete the first cycle and this action repeats continuously.

\textbf{Second scenario (deterministic requirement):} In this case, we assume a non-probabilistic configuration of the first scenario where $i^{th}$ ($i \in 1, 2, ..., D$) drone starts to take off from the neighborhood area center at time $T_i$ ($T_i \in (0,\tau)$) which is defined by Equation (\ref{eq:Tnonrandom}). In this case, the houses are distributed uniformly over the neighborhood edge and packages are sent to houses uniformly.  

%It picks up a package $x_i = k$, where $i = 1, 2, ...$, and $k$ is uniformly distributed over $1, 2, ..., N$, and flies to a predetermined altitude of $H$.  Then it flies in a straight line with angle $\theta_k$, which is uniform over $(0, \theta_{max})$, towards the neighborhood edge. When the drone reaches the destination and delivers its package, it returns to the origin on the same angle and this action repeats continuously.
\begin{equation} \label{eq:Tnonrandom}
T_{i}=\frac{i}{D+1}\tau
\end{equation}

\textbf{Third scenario (non-uniform distribution of houses):} In this case, we consider $D$ drones with take off time $T_1, T_2, ..., T_D$, which are uniformly distributed over $(0, \tau)$. We assume houses are distributed non-uniform over the neighborhood edge. It means that their angles $\theta_1, \theta_2, ..., \theta_D$ have a non-uniform distribution over $(0, \theta_{max})$.  Packages are sent to houses uniformly. We consider two models for this scenarios which are explained in detail in Section~\ref{sec:algorithm}. 

%Each drone first picks up a package $x_i = k$, where $i = 1, 2, ...$, and $k$ is uniformly distributed over $1, 2, ..., N$, and flies to a predetermined altitude of $H$. Then it flies in a straight line with angle $\theta_k$, which is non-uniform over $(0, \theta_{max})$, towards the neighborhood edge. When a drone reaches its destination house and delivers its assigned package, it returns to the origin on the same angle to complete the first cycle and this action repeats continuously. We define two models for this scenarios which are explained in detail in Section~\ref{sec:algorithm}.

\textbf{Fourth scenario (The most general scenario):} In a practical scenario, we consider $D$ drones with take off time $T_1, T_2, ..., T_D$, which are uniformly distributed over $(0, \tau)$. We assume houses are distributed non-uniformly over the neighborhood edge, and the packages are sent to them non-uniformly, too. This scenario is more practical because in reality, the packages are sent to some houses more than other houses and there are vary density houses in the different location of neighborhood area. We propose two algorithms for this scenario which we explain in Section~\ref{sec:algorithm}. 
% in a non-uniform distribution for the package destinations which means $X_1, X_2, X_3, ...$ are not uniformly distributed over $1, 2, ..., N$. So in this case, each drone first picks up a package $x_i = k$, where $i = 1, 2, ...$, and $k$ is not uniformly distributed over $1, 2, ..., N$. Then it flies in a straight line with angle $\theta_k$, which is uniformly distributed over $(0, \theta_{max})$, towards the neighborhood edge. When a drone reaches its destination house and delivers its assigned package, it returns to the origin on the same angle to complete the first cycle and this action repeats continuously. We define two algorithms for this scenarios which we explain them in Section~\ref{sec:algorithm}. 

In the next section, we show that for all scenarios at any snapshot of $t$, once all $D$ drones are on air, they can provide uniform network coverage, and at the same time, they can provide package delivery with high efficiency.
   
















































